CFP: Efficient Optimization of Intra-Operator Parallelism Plans for Large Model Training

Optimizing the parallel training of large models requires exploring intra-operator parallelism plans for a computation graph that typically contains tens of thousands of primitive operators. While the optimization of parallel data processing graphs has been extensively researched in database systems, the vast search space makes it challenging to apply traditional database query optimization methods and algorithms. This paper introduces CFP, an optimization system for intra-operator parallelism that significantly reduces the complexity of searching for parallelism plans by leveraging two structural patterns found in large models. First, we identify parallel-preserving subgraphs, which ensure that the optimal global plan assigns the same parallel strategy to all operators within the subgraph. This approach allows us to avoid enumerating all possible combinations of parallel strategies for these operators. Second, we recognize repetitive subgraph patterns within the large computational graph, enabling us to profile a moderate number of representative subgraphs and accurately estimate the cost of parallelism plans with low overhead. With the significantly reduced search space, we can employ dynamic programming to search for the optimized parallelism plan. In our experiments, we demonstrate that CFP achieves significant speedups compared to the state-of-the-art framework for large models like GPT and LLAMA.

==> CFP-VLDB-arxiv-v2/content/Background.tex <==
\vspace{-1ex}
\section{Background and Motivation}\label{background_motivation}

\begin{figure*}
    \centering
    \includegraphics[width=0.98\textwidth]{fig/motivation_example_250512.png}
    \vspace{-3mm}
    \caption{Parallelism strategies for MatMul and two parallelism plans for a Transformer layer. After code lowering and optimizations, there is a noticeable mismatch between the actual communication workloads and the theoretical cost. }
    \vspace{-4mm}
    \label{fig:motivation}
\end{figure*}

% \subsection{Intra-operator Parallelism Plan}
\subsection{Parallelism Strategy for Operators}

%Deep learning model training consists of two main phases: a forward pass, which computes intermediate activations and final outputs by applying the model's parameters to the input data, and a backward pass, which computes the gradient of the loss with respect to each model parameter, indicating how the parameters should be adjusted to reduce the loss.
%These computations are typically represented by a Data Flow Graph (DFG), also known as a computation graph, which captures the sequence of operations applied to multi-dimensional tensors. 


Model training involves a forward pass, which computes intermediate activations by applying the model's parameters to the input data, and a backward pass, which computes the gradient of the loss with respect to each parameter.
These computations are typically represented by a computation graph, which captures the sequence of operations applied to multi-dimensional tensors. 


Operators in the computation graph can be broadly categorized into three types:
(1) Tensor contraction operators, such as matrix multiplication (MatMul) and reduce. These operators are typically compute-intensive and often change the shape of tensors by reducing or expanding specific dimensions.
(2) Element-wise operators, such as addition, subtraction, and multiplication, which apply the same operation independently to each tensor element.
(3) Data manipulation operators, such as reshape and transpose, which change the layout or shape of tensors. 
% Each node in the graph corresponds to a operator, and each edge represents a tensor flowing between operators.
% For an operator $f: X \rightarrow Y$, where $X \in \mathbb{R}^{d_{1} \times \cdots \times d_{k}}$ and $Y \in \mathbb{R}^{d'_{1} \times \cdots \times d'_{l}}$,
% a \textit{parallelism strategy} specifies how the multi-dimensional input and output tensors of the operator are partitioned across devices and how the computation is distributed accordingly.
% Formally, it specifies two subsets of tensor dimensions, $P_{\text{X}} \subseteq \{1, \dots, k\}$ and $P_{\text{Y}} \subseteq \{1, \dots, l\}$, which are used to shard the input and output tensors, respectively.
% Each selected dimension is associated with a group of devices, and data along that dimension is split accordingly, resulting in \textit{parallel partitions}, i.e., independent data slices assigned to individual devices for local computation.

In intra-operator parallelization, operators are executed on target devices in a SPMD  fashion.
These devices are typically organized into a logical \textit{device mesh}, where they are arranged into a multi-dimensional grid.
% These devices are organized into a logical \textit{device mesh}, a multi-dimensional grid.
For example, 8 GPUs on a node can be organized as a $1 \times 8$ mesh with a single axis, or as a $2 \times 4$ mesh with two axes.
% Based on this, for an operator $f: X \rightarrow Y$: $X \in \mathbb{R}^{d_{1} \times \cdots \times d_{k}}$ and $Y \in \mathbb{R}^{d'_{1} \times \cdots \times d'_{l}}$, a \textit{parallelism strategy} specifies how to partition its input and output tensors over the device mesh and how to distribute the computation accordingly.
% Formally, it specifies two subsets of tensor dimension indices, $P_{\text{X}} \subseteq \{1, \dots, k\}$ and $P_{\text{Y}} \subseteq \{1, \dots, l\}$, indicating which dimensions of the input and output tensors are mapped to axes of the device mesh.
Based on this, for an operator $f: X \rightarrow Y$: $X \in \mathbb{R}^{d_{1} \times \cdots \times d_{k}}$ and $Y \in \mathbb{R}^{d'_{1} \times \cdots \times d'_{l}}$, a \textit{parallelism strategy} specifies how to partition its input tensors over the device mesh and how to distribute the computation accordingly.
Formally, it specifies a subsets of tensor dimension indices, $P_{\text{X}} \subseteq \{1, \dots, k\}$, indicating which dimension of the input tensor are mapped to each axis of the device mesh.
The data along each mapped tensor dimension is then partitioned across the set of devices along the corresponding mesh axis.
As a result, the input and output tensors are divided into \textit{parallel partitions}, i.e., data slices assigned to individual devices for local computation.
If $P_{\text{X}}$ is empty, the input tensor is not partitioned and is instead fully replicated across the devices.
% The choice of $P_{\text{X}}$ and $P_{\text{Y}}$ is constrained by the operator's data dependency structure, i.e., how each output dimension is computed from input dimensions.

Given the input partition dimensions, the partitioning of an operator's output tensor is constrained by its semantics and the data dependencies between input and output.
Therefore, we refer to the input dimensions in $P_{\text{X}}$ as the operator’s \textit{parallel dimensions}, as they determine how data and computation are partitioned across devices.
% Due to the data dependencies of the operator, these input-side parallel dimensions induce a corresponding $P_{\text{Y}}$ on the output tensor.
When an operator has multiple inputs and outputs, the definition naturally extends by assigning parallel dimensions to each input and output tensor individually.
Moreover, the parallel dimensions across multiple input tensors must be chosen compatibly, so that the operator can be correctly executed on partitioned data without violating operator's semantics.


% The communication behavior under parallelism varies across operator types: tensor contraction may require synchronization if parallelizing reduction dimensions; data manipulation operators can trigger collective communication (e.g., all-to-all) when their layout transformations conflict with partitioned dimensions; while element-wise operators, by their element-independent nature (one-to-one mapping), inherently avoid communication.
% The communication behavior under parallelism varies across operator types: 
% Tensor contraction operators may require communication when parallelizing certain tensor dimensions. 
% Specifically, if the partitioned tensor dimensions are involved in data reduction (e.g., summing or averaging), the output must be collected from different devices to produce correct results.
% Data manipulation operators can also trigger communication, as transforming data layout may require data from other devices under a given tensor partitioning, necessitating data exchange across devices;
% while element-wise operators, by their element-independent nature (one-to-one mapping), inherently avoid communication between parallel instances.

Taking matrix multiplication in Fig.~\ref{fig:motivation}(a) as an example, the operator 
$f: (A, B) \mapsto C$, where $A \in \mathbb{R}^{M \times K}$, $B \in \mathbb{R}^{K \times N}$, and $C \in \mathbb{R}^{M \times N}$ 
performs a tensor contraction along the shared dimension $K$ and can be parallelized by selecting different parallel dimensions from the input tensors $A$ and $B$.
Specifically, there are three commonly used parallelism strategies:
(1) Row-wise parallelism: choose $P_A = \{1\}$ (the $M$ dimension of $A$) and $P_B = \emptyset$. Each device holds a subset of rows of $A$ and the full $B$, and computes a corresponding row block of $C$.
(2) Column-wise parallelism: choose $P_A = \emptyset$ and $P_B = \{2\}$ (the $N$ dimension of $B$). Each device holds a subset of columns of $B$ and the full $A$, and computes a corresponding column block of $C$.
(3) Split-K parallelism: choose $P_A = \{2\}$ and $P_B = \{1\}$ (the shared $K$ dimension).
Each device holds slices of $A$ and $B$ along the reduction dimension and computes partial results for $C$, which are then aggregated via an inter-device communication (e.g., All-Reduce) to produce the final output.

% These strategies reflect different choices of parallel dimensions for the inputs, and induce corresponding data layouts and communication patterns.
% In particular, parallelizing along reduction dimensions typically incurs communication overhead to aggregate partial outputs, whereas partitioning along non-reduction dimensions can avoid synchronization and enable fully local computation.

\subsection{Intra-operator Parallelism Plans}

An \textit{intra-operator parallelism plan} is the global assignment of parallelism strategies to all operators in the computation graph, collectively determining the overall pattern of computation and inter-device communication.
When a tensor produced by one operator is consumed by another, their parallelism strategies may be incompatible, i.e., they partition the shared tensor along different dimensions.
Such mismatches require resharding of the tensor at operator boundaries, introducing inter-device communication.
Therefore, the choice of parallelism strategies not only affects local computation but also determines the global communication pattern.

Fig. \ref{fig:motivation}(b) shows a simplified Transformer layer, where an input tensor is first multiplied by a parameter matrix, then processed by a self-attention block, and finally multiplied by another parameter matrix. 
By adjusting the parallelism strategies assigned to the two MatMuls, we obtain two widely used intra-operator parallelism plans. 
On the left, both MatMuls adopt a row-wise parallelism strategy, allowing each device to independently compute on separate input data using a replica of the model parameters. 
During training, the gradients computed for parameters on each device must be synchronized to ensure consistent parameter updates across all replicas, thereby forming data parallelism.
On the right, the first MatMul adopts column-wise parallelism strategy, while the second MatMul uses split-K parallelism.
Each device produces a full-sized output tensor, but its element values are only partial results.
The partial results must be communicated immediately to assemble the full tensor before the next computation stage. 
This forms tensor parallelism plan, where communication is embedded within the forward and backward passes to maintain correctness.

% On the left, both matmuls are row-partitioned on the input tensor, enabling communication-free forward execution but requiring gradient synchronization after the backward pass, thereby forming data parallelism.
% On the right, column-wise partitioning of the first matmul’s parameters and reduction-dimension partitioning of the second matmul correspond to tensor parallelism, necessitating immediate inter-device reduction of the output tensor to ensure correctness.


Automatically generating such intra-operator parallelism plans is challenging, as it requires selecting a parallelism strategy for each operator, leading to a massive search space in large models.
This forces existing frameworks to build simplified symbolic cost models and adopt efficient search algorithms to find good solutions within a reasonable time.
For example, communication cost is typically estimated by the number of bytes derived from the shape and data type of the communicated tensors, while computation cost is measured by the number of floating-point operations required by each operator.

% \subsection{Theoretical vs. Actual Overheads}\label{motivation_example}

% First, the execution efficiency of a parallel configuration can be significantly affected by downstream compilation and optimization techniques~\cite{astitch, unity2022}. For example, compilers may automatically fuse multiple operators to improve computation and communication efficiency~\cite{nsdi22_optimize_comm_for_dp, icdcs23_opt_all_reduce}.  Second, the runtime dynamic selection of communication algorithms and their hardware-dependent implementations further increase performance uncertainty. For instance, the actual performance of the underlying communication library is highly sensitive to the runtime tensor size~\cite{asplos22_synthesis_comm_kernel, nsdi23_taccl_comm_library}.  These unpredictable performance characteristics severely undermine the reliability of static cost models. While it is theoretically possible to include all these factors into a symbolic cost model or use an ML-based model to account for them, such a model would be overly complex and extremely sensitive to subtle variations in the target runtime environment.

In practice, there is a substantial gap between the cost estimated by the symbolic model and the actual performance produced during execution.
% First, the execution efficiency of a parallelism plan can be significantly affected by downstream compilation and optimization techniques~\cite{astitch, unity2022}. For example, compilers may automatically fuse multiple operators to improve computation and communication efficiency~\cite{nsdi22_optimize_comm_for_dp, icdcs23_opt_all_reduce}.  
% Second, the runtime dynamic selection of communication algorithms and their hardware-dependent implementations further increase performance uncertainty. 
% For instance, the actual performance of the underlying communication library is highly sensitive to the runtime tensor size~\cite{asplos22_synthesis_comm_kernel, nsdi23_taccl_comm_library}.  
% These unpredictable performance characteristics severely undermine the robustness of static cost models. 
% While it is theoretically possible to include all these factors in a symbolic cost model or use an ML-based model to account for them, such a model would be overly complex and extremely sensitive to subtle variations in the target runtime environment.
Consider data and tensor parallelism for the transformer layer in Fig.\ref{fig:motivation}(b).
Given a \textit{hidden\_size} of 5120, \textit{seq\_len} of 1024, and \textit{batch\_size} of 16, Alpa~\cite{zheng2022alpa} estimates the cost of each parallelism plan by theoretically analyzing the communication data volume on the computation graph. 
It produces cost values of $1.51 \times 10^9$ for the tensor parallelism plan and $1.89 \times 10^9$ for the data parallelism.
However, the actual communication overhead diverges significantly from the theoretical communication volume-based cost. 
As shown in Fig.~\ref{fig:motivation}(c), tensor parallelism incurs extra overhead due to a compiler restriction that forces RNG operators to run on a single GPU. This requires an additional communication step to broadcast random data to other GPUs.
In contrast, data parallelism benefits from fusing communication for gradients of multiple parameters into a single, more efficient All-Reduce.
On 4 A100-PCIe GPUs, the communication time of data parallelism is only 60\% of that of tensor parallelism, despite its higher theoretical cost. This highlights the need to estimate cost based on the physical execution plan produced by the compilation and runtime system.

This gap arises because existing frameworks must efficiently search over a massive parallelism space, which forces them to rely on static analysis on the computation graph.
We observe that these frameworks overlook two types of important structural information, which are crucial for reducing search complexity. 
By exploiting these structural properties, we can extract a small set of representative parallel programs and profile them to estimate the costs of physical execution plans.
%Inspired by sampling-based query optimization, we exploit such structures to extract a small set of representative parallel programs. 
%We then profile these programs to estimate the cost of physical execution plans.
To explore this idea, we develop \sysname, a profile-based automatic intra-operator parallelism search system.

% In this paper, we observed that these frameworks 
% overlook two types of important structural information, which are crucial for reducing search complexity.
% By exploiting such structures, we can extract a set of representative structures and perform accurate performance evaluation on them. 
% This avoids the need to exhaustively evaluated all operator combinations using symbolic cost models.
\vspace{-1mm}
\subsection{System Overview}
% Inspired by sampling-based query optimization in database systems, 
% we estimate the cost of the physical intra-operator parallelism plans by profiling small representative parallel programs, instead of relying on static analysis on the computation graph.
% To explore this idea, we developed \sysname, a profile-based automatic intra-operator parallelism optimization system.

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{fig/overview_0701.png}
    \vspace{-7mm}
    \caption{System Overview}
    \vspace{-5mm}
    \label{fig:overview}
\end{figure}


\sysname performs its analysis and optimization on the XLA compiler’s intermediate representation. 
It uses the compiler frontend to convert the model into a computation graph, and uses the backend and XLA runtime to generate and profile the representative programs. 

Fig.~\ref{fig:overview} shows the system overview of \sysname. 
\textbf{\textcircled{1}} After the compiler frontend translates the model into a static single assignment (SSA) form, it produces a linearized sequence of primitive operators.
\sysname analyzes element-level data dependencies between operators to identify subgraphs with parallelism-preserving properties. 
It then groups the corresponding operators into {\pb}s, which serve as basic units for constructing the parallelism search space, i.e., combining the parallelism strategies of multiple {\pb}s within the model or model segment to form a global or sub-parallelism search space.
%
\textbf{\textcircled{2}} \sysname treats the entire graph as a sequence of {\pb}s and applies template matching to extract a set of distinct subsequences (model segments). 
It extracts the element-level dependency graph of tensor contraction operators from the subsequences, which is used as a fingerprint for matching with other subsequences. 
This approach ensures that the matched subsequences share the same sub-parallelism space and parallel execution behavior, while significantly reducing the complexity of segment matching.
%
\textbf{\textcircled{3}}\sysname profiles each distinct model segment separately by building and running all plans in its sub-search space, collecting the computation and communication overhead, as well as memory consumption for each plan.
In addition, it also profiles the cost of tensor resharding across neighboring {\pb} pairs when there are mismatches between the output tensor partition of one segment and the input partition expected by the next.
%
\textbf{\textcircled{4}} It reuses the profiling results to estimate the execution cost of all matched segments, as well as the overhead of cross-segment tensor resharding. 
Subsequently, it aggregates these estimates to compute the overall execution cost and memory consumption of each global parallelism plan.
%
\textbf{\textcircled{5}} It uses a dynamic programming algorithm to find the optimal parallelism plan while satisfying the memory limit of the target platform.
The plan is then passed to the compiler backend to generate the final intra-operator parallel program.


==> CFP-VLDB-arxiv-v2/content/Conclusion.tex <==
\section{Conclusion}
%\sysname currently does not consider multi-dimensional partition and temporal dimension partition. 
%These partitioning methods further expand the tensor parallel search space and may lead to higher computation and communication efficiency.
%Our future work will focus on using profile-based methods to identify multi-level parallel plans, including pipeline parallelism, seeking end-to-end parallel training solutions for large models that closely align with optimal real-world performance while maintaining reasonable search time.

This paper introduces \sysname, a system that search intra-operator parallelism configurations by leveraging runtime profiles of actual parallel programs. 
The key idea is to profile a limited space by identifying a new structure named \pb, which is a group of operators enjoying communication-free tensor partition propagation.
An optimal tensor partition of operators within a \pb should be inferred from the partition of input tensor through partition propagation to avoid additional communication.
Thus, it is sufficient to profile each \pb with different input tensor partitions.
On GPT, LLAMA, and MoE models, \sysname achieves up to a 1.51x, 1.31x, and 3.43x performance improvement over the state-of-the-art framework, Alpa. 


==> CFP-VLDB-arxiv-v2/content/Evaluation/Analysis.tex <==

\vspace{-4mm}
\subsection{Communication Overhead Analysis}

We observed that most parallelism plans evenly distribute heavy operators across multiple GPUs, making communication overhead the main factor causing significant differences in final throughput, especially on the A100-PCIe platforms.
Fig.\ref{fig:bandwidth} shows the communication overhead and utilized communication bandwidth by the four frameworks on 4xA100-PCIe GPUs. 
%可以删掉
% PyTorch data parallelism relied on many inefficient reduce and scatter kernels for gradient synchronization and parameter updates, which resulted in low utilized communication bandwidth and high communication overhead. 
% Although Deepspeed-Megatron achieved higher utilized communication bandwidth, it relied on pre-defined parallel templates and failed to optimize communication workload, leading to suboptimal communication overhead. 
% In contrast, while Alpa always chooses the parallelism plan with the smallest theoretical communication volume, it is not aware of the actual compiled communication workload and efficiency, resulting in lower utilized communication bandwidth and higher communication overhead.
\sysname balanced communication volume and efficiency, achieving the smallest communication overhead across the four models.


\begin{figure}
    \centering
    \includegraphics[width=0.47\textwidth]{content/Evaluation/fig/comm_comp_cost_1211.png}
    \vspace{-4mm}
    \caption{Time of computation and communication kernels for plans in \sysname's intra-operator parallelism search space. Sorted in ascending order of Alpa's communication volume-based cost, with only the top 20 selected for clarity.}
    \vspace{-1mm}
    \label{fig:volume_and_overhead}
\end{figure}

We further investigated the discrepancy between the theoretical cost based on communication volume and the measured performance. 
As shown in Fig.\ref{fig:volume_and_overhead}, %illustrates the computation and communication kernel overhead for the top 20 plans with minimal theoretical cost in \sysname's search space.
while communication kernel overhead indeed increases with theoretical cost,
parallelism plans with similar theoretical cost can have significantly different communication overheads. 
For instance, in BERT, the 6th to 8th plans had similar theoretical costs, but their actual overheads differed by a factor of two. 
Moreover, plans with optimal communication overhead can have substantially higher theoretical costs, e.g., the parallelism plan (the 14th) with the highest efficiency in MoE had a theoretical cost 1.45 times that of the smallest cost.
We believe that two main reasons contribute to such a significant discrepancy:
(1) The unpredictable effects of code lowering and optimization: The compiler may generate unexpected communication kernels for certain communication patterns, or it may optimize the communication bandwidth through compiler optimization techniques. 
(2) The complex relationship between communication efficiency, target platform, communication algorithms, and tensor shapes: even with similar communication workloads, these factors can significantly affect the communication efficiency, leading to highly variable communication overhead.


%可以删掉
% \subsection{{Accuracy of the Profile-based Cost Model}}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.47\textwidth]{content/Evaluation/fig/predict_acc_250425.png}
%     \vspace{-4mm}
%     \caption{
%     Average training time per iteration and cost predictions by \sysname for GPT-6.7B with a batchsize of 16. }
%     \label{fig:cost_acc}
% \end{figure}

% \sysname's profile-based cost model predicted the performance by combining real-world training profiles. 
% It limited performance unpredictability of parallelism plans to a small range within the computation graph, i.e., at the connections between model segments. 
% % Fig. \ref{fig:cost_acc} shows the performance prediction results of \sysname for the GPT-6.7B model with different parallelism plans on two target platforms. 
% % To limit the number of parallel programs, model segments with the same fingerprint were assigned consistent plans.
% On the A100-PCIe platform, the root mean square error (RMSE) between the predicted costs and actual training time is 0.03286. 
% On the V100-NVLink platform, the higher utilized communication bandwidth compared to the PCIe platform results in a smaller proportion of cross-segment communication time to total training time, leading to more accurate performance predictions with an RMSE of 0.007885.



==> CFP-VLDB-arxiv-v2/content/Evaluation/CaseStudy.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.47\textwidth]{content/Evaluation/fig/casestudy_0322.png}
    \vspace{-4.5mm}
    \caption{Parallelism plans searched by Alpa and \sysname for MoE-7.1B batchsize 16 and LLAMA-7B batchsize 80. GATE, ATTN, and RNG stand for gated network, attention block, and random number generator operator, respectively. }
    \vspace{-1mm}
    \label{fig:case_study_1205}
\end{figure}

\vspace{-3.5mm}
\subsection{Case Study}

%We analyzed the parallelization of the MoE model on the A100-PCIE platform due to noticeable performance fluctuations with different Parallelism configurations. 
%On the NVLink platform, we analyzed the parallelization of LLAMA, as its communication bottlenecks are more apparent on high-bandwidth platforms. 

\textbf{GShard MoE on A100-PCIe.}
Fig.12(a)(b) shows the parallelism plans searched by Alpa and \sysname for a single MoE layer. Alpa partitions the data dimension of each operator and adopts ``expert parallelism'' for the expert network.
This requires All-to-All communication to reshard intermediate results before and after the expert network and All-Reduce to aggregate gradients.
\sysname selects different plans for different batch size: when the batch size is smaller than 96, it uses a tensor parallelism-like plan to partition the parameters of the expert network. 
This requires All-Gather to reshard tensors before the expert network and All-Reduce to aggregate results, where the All-Reduce operation is rewritten by the compiler into a Reduce-Scatter.
For larger batch sizes, \sysname partitions the batch data dimension for all operators.
Alpa overlooked this plan because it  overestimated the communication cost of the tensor resharding after expert network by 8 times compared to the actual communication workload in 16 GPUs training. 
We observed that the parallelism plans searched by Alpa incurred twice the communication overhead of \sysname for batch sizes smaller than 96 and over three times the overhead for larger batch sizes.

\textbf{LLAMA on V100-NVLink.} 
Fig.12(c)(d) shows the parallelism plans searched by Alpa and \sysname for LLAMA-7B with a batch size of 80.
Alpa partitions the batch dimension of input data in the self-attention part and then partitions parameters for the remaining operators to minimize communication volume. However, this causes each GPU to call the random number generator operator independently, leading the compiler backend to insert extra All-Reduce for random data synchronization. 
In contrast, \sysname partitions all operators along the batch dimension, leverages the compiler to merge all gradient synchronizations into a single communication kernel for better efficiency.
Moreover, due to the higher interconnect bandwidth between GPUs on the NVLink platform, computation overhead has a more critical impact on overall training time. 
We observed that frequent communication in Alpa’s plan introduced more data movement operators (concat and split), making its computation overhead about 10\% higher than \sysname.



==> CFP-VLDB-arxiv-v2/content/Evaluation/CompileOverhead.tex <==

\vspace{-1.8mm}
\subsection{Profiling Space and Search Overhead}
For BERT, GPT, and LLAMA, \sysname extracts two segments besides embedding/output layers: one for the first hidden layer and one for subsequent layers.
Although structurally identical, these segments have different fingerprints due to element-level dependency variations introduced during code lowering.
Each segment yields 4 {\pb}s. The first tensor contraction (matrix multiplication) in each has 3 candidate parallel dimensions, resulting in $3^4=81$ parallelism plans per segment. 
In addition, profiling is required for tensor resharding across segment boundaries and repeated segments, covering $3\times3=9$ groups of communication kernels. 
In total, $2 \times 81 + 2 \times 9 = 180$ programs are compiled and profiled.
% The profiling space of \sysname depends on the constructed {\pb}s and distinct model segments, as discussed in Sec.\ref{SearchSpace} and Sec.\ref{profling_method}.
% Besides the embedding and output layers, \sysname extracted two distinct segments from BERT, GPT, and LLAMA: one for the first hidden layer and another for each subsequent hidden layer.
% Despite having the same structure and tensor shapes, they have different fingerprints due to inconsistent fine-grained dependencies between tensor contraction operators after code lowering. 
% For each segment, it constructed 4 {\pb}s, with the first tensor contraction operator (matrix multiplication) in each \pb having 3 candidate parallel dimensions, resulting in $3^4=81$ parallelism plans per segment.
% Additionally, tensor resharding across the boundary between the two segments, from the last \pb of the first to the first \pb of the second, requires compiling and profiling $3*3=9$ groups of communication collective kernels.
% Similarly, since the second segment is repeated multiple times, resharding between its first and last \pb also requires profiling 9 groups of communication collective kernels.
% Additionally, tensor resharding between segments needs to be profiled. Specifically, resharding occurs across the boundary between the two distinct segments and within repetitions of the second segment, requiring $3\times3=9$ groups of communication collective kernels for each case.

For MoE models, \sysname treats alternating MoE and Transformer blocks as separate segments, each with 4 {\pb}s.
One \pb in MoE blocks involves batched matrix multiplication with an additional expert-related batch dimension, increasing its candidate dimensions and slightly expanding the profiling space.
% For MoE, \sysname treats the alternating MoE blocks and Transformer blocks as separate segments, constructing 4 {\pb}s for each.
% In MoE blocks, one \pb's first tensor contraction operator is a batched matrix multiplication, with the additional batch dimension corresponding to the experts. 
% This adds an extra candidate parallel dimension to this \pb compared to others, resulting in a slightly larger profiling space for the MoE model than other models.

%可以删掉
% For the profiling space of 2D parallelism plans, we enforces mapping the data batch dimension of each \pb to the multiple GPU nodes, while GPUs within a single node can parallelize along any data dimension. 
% This restricts the profiling space of 2D parallelism plans to the same size as that of 1D parallelism plans.

\sysname's search overhead can be divided into four parts. 
\textit{AnalysisPasses}, refers to constructing {\pb}s and extracting distinct segments for model. 
\textit{ExecCompiling} represents the overhead of compiling and generates all executable programs that need to be profiled. 
\textit{MetricsProfiling}, refers to the overhead involved in running these programs multiple times to collect profiles.
\textit{ComposeSearch}, represents the cost of combining the profiling results of distinct segments to search for the globally optimal parallelism plan.

The magnitude of \textit{ExecCompiling} depends on the number of distinct segments and the parallelism space of each segment. 
\textit{MetricsProfiling} is influenced by the training workload of each plan.
Fig. \ref{fig:search_overhead} shows these two overhead details for GPT-2.6B, MoE-7.1B, and LLAMA-7B. 
As the batch size increases, the \textit{ExecCompiling} remains relatively stable, while \textit{MetricsProfiling} increases. 
By parallelizing the compilation, overlapping it with the profiling process, and using a dynamic profiling time budget, \sysname significantly reduced the search overhead by trimming inefficient or stalled parallelism plans, as shown by \textit{OptimizedOverall} in Fig. \ref{fig:search_overhead}.

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{content/Evaluation/fig/cfp/vldb_new_compile_overhead.png}
    \vspace{-7.5mm}
    \caption{Compiling and profiling time for distinct segments in three models on a platform with 4 A100-PCIe GPUs.}
    \vspace{-5.5mm}
    \label{fig:search_overhead}
\end{figure}


The overhead of \textit{AnalysisPasses} and \textit{ComposeSearch} is not affected by the training workload but increases as the model depth grows. We evaluated the overhead of them with different numbers of hidden layers on three models, as shown in Fig.\ref{fig:analysis_overhead}. In most intra-operator parallelism exploration scenarios (e.g., searching for parallelism plans inside a pipeline stage), their overhead is much smaller than \textit{ExecCompiling} and \textit{MetricsProfiling}.

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{content/Evaluation/fig/cfp/vldb_new_analysis_overhead.png}
    \vspace{-7mm}
    \caption{Analyzing and searching time for different numbers of layers of three models with a 24-core processor.}
    \vspace{-1mm}
    \label{fig:analysis_overhead}
\end{figure}

\vspace{-1.8mm}
\subsection{Scalability Analysis}\label{scalability}

For larger systems with more GPUs, there are two typical cases where \sysname can be used with no increase in analysis and profiling complexity.
(1) Combine \sysname with data parallelism to exploit multi-dimensional intra-operator parallelism. Suppose the model is trained using data parallelism across multiple worker groups. \sysname can be applied in each group using its original workflow, and its profiles can be reused across all groups. 
(2) Combine \sysname with pipeline parallelism. \sysname can explore intra-operator parallelism within each potential pipeline stage, where the profile results of model segments (smaller than a stage) can also be reused for stage profiling to determine the best pipeline stage partitioning. 

For larger models, \sysname's profiling space will not increase unless there are new distinct segments. 
More layers may raise \sysname’s analysis and search overhead, and increasing configuration settings like hidden size may raise the profiling overhead for distinct segments. However, these overheads remain negligible compared to the training time.
While the complexity of the final search process increases nonlinearly with the number of layers, it is possible that future models with extremely deep architectures make dynamic programming infeasible. In such cases, techniques from database query optimization (e.g., genetic algorithms) can be employed while still leveraging physical execution costs to guide the search.

% We built {\pb}s and model segments for LLAMA3.1-405B and profiled its unique segments on an 8xA100-PCIE GPU node. We observed that the overheads were still acceptable: For 32 llama layers (8B) to 126 layers (405B), the analysis overhead increased from 26 seconds to 235 seconds, and the profiling overhead increased from 117 seconds to 463 seconds for batch size of 32. In fact, the profiling overhead could be reduced further if more nodes were available for profiling.




==> CFP-VLDB-arxiv-v2/content/Evaluation/E2EPerf.tex <==

\vspace{-2mm}
\subsection{Training Performance}

Although \sysname significantly reduces the intra-operator parallelism search space, the reduced space still includes the data parallelism plan, the tensor parallelism plan, and the communication volume-optimal plans searched by Alpa. 
However, \sysname may not select these solutions as they might not achieve the best profile-based cost.
Fig. \ref{fig:e2e_perf_1201} shows the average throughput achieved by four parallel frameworks on two platforms. 
PT and DS-M utilize fixed parallel templates, which makes it challenging to achieve optimal throughput across all training settings. 
This limitation is even more significant for models that require more flexible parallelism plans, such as LLAMA and MoE models, leading to larger performance gaps between fixed parallel templates and optimized plans.

\sysname achieved an average performance speedup of 1.17x over Alpa with 4 GPUs and 1.63x with 8 GPUs.  
We observed that Alpa's communication volume-based cost model lacked awareness of downstream compilation and the efficiency of communication primitives, leading to inaccurate predictions of communication workload and efficiency in many experimental settings.  
For GPT and LLAMA, Alpa searched a tensor parallelism-like plan to minimize communication volume in transformer layers for small batch sizes.  
This introduced unexpected communication workloads during downstream compilation, offsetting the benefits of minimizing theoretical communication volume.  
In contrast, \sysname partitioned batch dimensions for each operator in these settings, achieving higher communication efficiency after All-Reduce kernel fusion and up to 1.51x and 1.31x speedup over Alpa on the two models, respectively.



For GShard MoE, \sysname achieved an average performance speedup of 2.13x over Alpa. 
Although Alpa's parallelism plan has the optimal communication volume, the compiled parallel program relies on multiple inefficient ncclSendRecv kernels on PCIe platforms. 
In contrast, \sysname used a hybrid parallelism plan: it splits batch dimensions for most operations but splits different dimensions for operators in the expert network, depending on the batch size. 
These parallelism plans rely on more efficient collective communication primitives, such as All-Gather and Reduce-Scatter. 


\textbf{Multiple A100-PCIe Node.} 
We evaluated 4 frameworks on a 16-GPU cluster arranged as 1D and 2D device meshes (1×16, 2×8, 4×4), enabling hierarchical parallelism: one parallel dimension across nodes, another within nodes.
We used Alpa to explore the full space, while \sysname restricts the data batch dimension to the outermost mesh axis to keep the search space consistent with the 1D case.

A more complex communication topology makes it harder for Alpa's cost model to evaluate the performance of different parallelism plans accurately. 
It struggled to evaluate communication spanning multiple device levels, such as collective communication involving both inter-node and intra-node. 
As a result, even though its search space includes both 1D and 2D intra-operator parallelism plans, it overlooks 1D plans in many cases, even when those could provide better communication efficiency.

Moreover, multi-level communication provides the compiler with more optimization opportunities, making the actual communication workload deviate even more from the theoretical cost. 
For example, \sysname employs tensor parallelism for the expert network part in MoE. 
This requires All-Gather and All-Reduce for data aggregation before and after the expert network.
In practice, this plan results in less communication time because the compiler's downstream optimization automatically rewrite multiple communication kernels into more efficient ones with reduced communication volume.
However, Alpa overlooked this plan because its estimation of the resharding communication cost was 8x higher than the actual communication workload.
\sysname avoids these issues by profiling real-world communication costs, achieving a maximum speedup of 2.01x on BERT, 1.43x on GPT, 3.06x on MoE, and 1.67x on LLAMA.

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{content/Evaluation/fig/cfp/bandwidth_cfp.png}
    \vspace{-10mm}
    \caption{Overhead and achieved bandwidths of communication kernels for four models with batchsizes of 8, 8, 32, and 80, respectively. A logarithmic scale was used for communication overhead. }
    \vspace{-1mm}
    \label{fig:bandwidth}
\end{figure}


\textbf{Single V100-NVLink Node.} 
With the higher inter-GPU communication bandwidth provided by the NVLink platform, the proportion of communication time in the overall training time is reduced.
Since the main performance differences between parallelism plans arise from differences in communication patterns, the reduced communication overhead narrows the overall performance gap between different plans.
As shown in Fig.\ref{fig:e2e_perf_1201}, compared to PT, DS-M, and Alpa, \sysname achieved average speedups of 1.73x, 1.61x, and 1.05x.
For MoE, both \sysname and Alpa found plans that reduced communication time to about 1/20 of the total training time, leading to no significant performance differences.
For other models, Alpa applies the same parallelism plans as those selected for the PCIe platform.
In contrast, \sysname identified optimal parallelism plans based on the profiles from the NVLink platform.











==> CFP-VLDB-arxiv-v2/content/Evaluation/MemConstraint.tex <==
\vspace{-1.8mm}
\subsection{Performance Under Memory Constraints}

\begin{figure}
    \centering
    \includegraphics[width=0.49\textwidth]
    {content/Evaluation/fig/cfp/mem_constraint_0630.png}
    \vspace{-7.5mm}
    \caption{Training performance of LLAMA-7B with different hidden layer numbers and batch sizes. Left: Fixed hidden layer number to 6, increasing batch size. Right: Fixed batch size to 128, increasing the hidden layer number.}
    \label{fig:perf_mem_constraint}
    \vspace{-1mm}
\end{figure}

We evaluated the parallel training throughput of \sysname under memory constraints on four A100-40GB GPUs.
Fig.~\ref{fig:perf_mem_constraint} shows the throughput of different parallel frameworks for training the LLAMA2 model with varying numbers of hidden layers and batch sizes.
Alpa chose parallelism plans without integrating memory constraints into the search process, which quickly led to out-of-memory problems as batch sizes and the number of hidden layers increased. 
We also compared \sysname with ZeRO stage-1\cite{zero20sc}, a state-of-the-art memory optimization framework. 
It distributes all optimizer states across each GPU, reducing memory usage but suffering from high communication costs, which results in lower throughput.

\sysname balanced throughput and memory usage by selecting different parallelism plans for different segments, enabling the training of deeper models than Alpa while achieving higher throughput than ZeRO stage-1.
Note that \sysname inevitably prunes many memory-efficient plans, such as FSDP, which results in its memory optimization having a lower upper limit compared to ZeRO.



==> CFP-VLDB-arxiv-v2/content/Evaluation/Setup.tex <==
\vspace{-1mm}
\section{Evaluation}

\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth]{content/Evaluation/fig/cfp/overall_vldb_0327.png}
    \vspace{-10mm}
    \caption{The average training throughput achieved by four parallel frameworks on two platforms.}
    \label{fig:e2e_perf_1201}
    \vspace{-5mm}
\end{figure*}


\sysname is an optimization system based on the Tensorflow-XLA framework.
We implemented optimization passes in the XLA compiler to build {\pb}s and extract distinct model segments. 
We also used the XLA compiler backend and runtime for generating and profiling SPMD programs. 
\begin{comment}
    
Our experiment aimed to answer the following questions: 
%\begin{enumerate}

(1) Does \sysname's reduction for parallelism search space limit its optimization opportunities, i.e., preventing it from achieving competitive performance?

(2) Can \sysname's profile-based cost model predict actual performance more accurately than symbolic cost model?

(3) How different are the predictions from the symbolic cost model and actual performance, and the causes?

(4) How much profiling workload is required in \sysname, and how long does the searching process take? 
%\end{enumerate}

\end{comment}

%To answer these questions, 
We compared \sysname with three parallel training frameworks: PyTorch (PT), DeepSpeed-Megatron (DS-M), and Tensorflow-Alpa (Alpa).
PyTorch employs data parallelism plans, which can be considered as intra-operator parallelism plans that split the batch dimension for all operators.
DeepSpeed-Megatron offers a manually designed parallel framework that incorporates both data and tensor parallelism. 
Alpa is one of the state-of-the-art automatic parallel frameworks that comprehensively considers inter-operator and intra-operator parallelism.
Its intra-operator parallelism search space contains parallelism plans equivalent to both data parallelism and tensor parallelism.
As Alpa's optimal solution for multi-level parallelism relies on the optimal intra-operator parallelism plan for each model segment (pipeline stage), we extracted its intra-operator parallel framework to compare with \sysname.
We believe that comparing with Alpa is appropriate, as its intra-operator search process has been widely adopted by newer parallel frameworks, such as nnScaler~\cite{nnscaler}, while also supporting more recent models than other automatic intra-operator parallel frameworks like FlexFlow~\cite{lu2017flexflow}.

\vspace{-2mm}
\subsection{Evaluation Setup}
We used four models in the evaluation: BERT~\cite{devlin2019bert}, GPT~\cite{gpt2020}, GShard MoE~\cite{GShardMoE} and LLAMA-2~\cite{touvron2023llama}. 
We set the micro batch size from 2 to 32 per GPU and report the average floating-point operations per second (FLOPS) during training.
\sysname can handle other models besides the evaluated ones because the construction of \pb{}s and distinct model segments is based on compiler IR.

During profiling of each distinct segment’s parallelism plan, we first ran the parallel program 5 times for warm-up, followed by 10 runs to collect the desired profile items. 
For the evaluation of the selected parallelism plan, we ran the test program 100 times and reported the average FLOPS.
We evaluated \sysname on two GPU nodes, each with 8 NVIDIA A100 40GB GPUs connected via PCIe. 
We also evaluated it on a node with 4 NVIDIA V100 16GB GPUs connected via NVLink to validate its optimization in the target platform with higher communication bandwidth.
On the A100-PCIe platform, all models are trained with TF32 precision, while on the V100-NVLink platform, we use FP16 precision due to memory constraints. 






==> CFP-VLDB-arxiv-v2/content/Introduction.tex <==
\section{Introduction}\label{intro}

%-----------background-----------
Recent advances in large models have propelled remarkable progress in diverse fields~\cite{yang2023harnessing, kirillov2023segment, RN245}. 
These models, characterized by their extensive parameter sizes and computational requirements, necessitate the collaborative processing power of hundreds or even thousands of GPUs over extended periods. 
Recent efforts have extended the training of large models to over 10K GPUs~\cite{megascale, llama3}. 
This has made optimizing parallelism in large models a critical challenge. %necessitating the selection of appropriate parallelism plans among a large number of GPUs.


Motivated by the massive data scale and computational demands in large model training, modern training systems have widely adopted multi-level parallelism configurations: from coarse-grained or inter-operator parallelism~\cite{narayanan2019pipedream, huang2019gpipe, AdaPipe} where the model is partitioned into segments handled by different GPUs or GPU groups, to fine-grained or intra-operator parallelism where the computation within each operator is split across multiple GPUs.
\textcolor{black}{Intra-operator parallelism can be applied to the whole model or orthogonally to model segments in inter-operator parallelism, e.g., stages in pipeline parallelism.}
This paper focuses on automatically searching for
efficient intra-operator parallelism plans,
which is crucial for the end-to-end performance of large model training~\cite{auto-parallel-survey}.

\textcolor{black}{
Intra-operator parallelism involves partitioning the computation of each operator in the model across different devices and running them in a Single Program Multiple Data (SPMD) form to improve training throughput and reduce memory usage~\cite{tofu2019, hap_heter_gpu_spmd_eurosys24}.
For example, a two-dimensional matrix multiplication can be partitioned by rows, columns, or reduction dimension, which exemplify an operator’s parallelization strategies, i.e., how a single operator’s computation is divided among multiple GPUs.
%
Each operator is assigned a parallelism strategy, and the combination of these individual strategies forms the overall parallelism plan of the entire model. 
Different intra-operator parallelism plans expose different communication and computation patterns, which can lead to significant differences in parallelism efficiency~\cite{xu2021gspmd}. 
}

Although manually designed intra-operator parallelism plan templates~\cite{li2020pytorch,megatronlm21sc,fsdp_pytorch}, such as tensor parallelism, data parallelism, or fully sharded data parallelism (FSDP), have achieved promising results, they require substantial development and tuning efforts~\cite {lepikhin2020gshardscalinggiantmodels}. 
A more general approach is to transform the model into a logical computation graph composed of primitive operators (e.g., matrix multiplication and arithmetic operations), and then automatically assign parallelism strategies to each operator to form a logical parallelism plan. Recent works have introduced many tensor partition abstractions for fine-grained operators~\cite{xu2021gspmd, santhanam2021distir, primpar_eurosys24}, thereby forming a comprehensive intra-operator parallel search
spaces~\cite{lu2017flexflow, zheng2022alpa, tofu2019}.

To quickly estimate the performance of different parallelism plans in the search space, most existing approaches adopt symbolic cost models based on static information. These models mainly consider the communication volume and the number of floating-point operations (FLOPs) required by each plan~\cite{zheng2022alpa, tofu2019, accpar, pase, cai2021tensoropt, D_rec}.
%Beyond symbolic models, 
Some other works explore machine learning-based models~\cite{icml17_rl_cost_model, gdp_rl_cost_model, lstm_cost_model, wang2020automap, lu2017flexflow} to capture the complex relationships among various factors and better model the impact of parallelism plans. 

These static models, whether symbolic or machine learning-based, primarily estimate the cost of parallelism plans of the logical computation graph. However, the logical computation graph must be compiled and optimized into a physical graph for execution. Consequently, the estimated cost often fails to align with the actual execution cost. For example, a compiler may automatically fuse multiple operators to optimize communication efficiency~\cite{nsdi22_optimize_comm_for_dp, icdcs23_opt_all_reduce}, resulting in a physical computation graph whose cost sufficiently deviates from that of the logical one.  
Furthermore, many factors of the runtime environment can increase the performance uncertainty. For instance, the actual performance of the underlying communication libraries is highly sensitive to the runtime tensor size~\cite{asplos22_synthesis_comm_kernel, nsdi23_taccl_comm_library}, partly due to their hardware-dependent optimization. These unpredictable performance characteristics severely undermine the reliability of static models. Incorporating all these factors into a static model would overly complicate the model, making it sensitive to subtle variations in the target runtime environment. 


To tackle these challenges, we can learn from query optimizers in database systems, which focus on estimating the cost of physical execution plans rather than logical plans. Additionally, to improve the robustness of the optimizer in uncertain execution environments, we draw inspiration from sampling-based query optimization~\cite{sampling_based_query}, which estimates the cost of query plans by executing queries on samples of data. More specifically, we propose a profiling-based method to robustly estimate the cost of the physical execution plan without requiring a priori knowledge of the actual compiler or execution environment. The idea is that the cost of each parallelism plan is estimated by compiling and running it on sampled data. However, simply borrowing the idea from database query optimizers will not work because the number of operators in a large model (e.g., on the order of tens of thousands) is typically much larger than that of a database query plan. Therefore, it calls for a much more efficient way to search and profile the parallelism plans of large models. Note that optimizing the parallelization of a computation graph has been proved to be NP-hard~\cite{partition_problem_nphard}. 

While the large number of operators in a computation graph leads to exponential growth in the parallelism plan space, we observe two key structural features that can be used to simplify the exponential plan space into a more manageable one, allowing for efficient and robust optimization of parallelism plans.



1) \textbf{Parallelism-preserving subgraphs.} 
A computation graph generally contains many subgraphs, within which all operators can be parallelized using the same strategy to eliminate the need for communication or synchronization between parallel operator instances caused by tensor re-partitioning.   We refer to such subgraphs as {\em parallelism-preserving} subgraphs.
We propose a new coarse-grained structural abstraction, termed \pb.
Each \pb contains a parallelism-preserving subgraph such that the optimal parallel plan would adopt a consistent parallelization strategy for all operators in the \pb.
Identifying parallelism-preserving subgraphs requires analyzing element-level data dependencies between operators, i.e., building the data mapping relations from source to destination at the tensor element level.
Since such dependencies are not directly available from the computation graph, we propose a novel method that constructs element-level dependencies between operators and identifies {\pb}s in a large computation graph efficiently. 
By collapsing all the operators within a \pb into one vertex, we can derive a significantly smaller computation graph. More importantly, our approach ensures that the reduced search space includes the globally optimal plan.


2) \textbf{Repetitive structural patterns.}
A large model typically consists of a limited number of repetitive structural patterns, e.g., identical layers repeated throughout the model. 
By identifying the repetitive structural patterns, we can extract and profile only a small set of representative subgraphs. 
Reusing the profiling results from these subgraphs enables us to estimate the cost of the entire model with significantly lower complexity while maintaining accuracy.
As the compressed graph remains very large (despite being significantly smaller than the original one), identifying the repetitive distinct patterns is computationally expensive. 
To solve this problem, we propose a novel mechanism to generate fingerprints of \pb sequences.
The fingerprint can be used to match different \pb sequences that share consistent sub-parallelism plan spaces and communication behavior.
As a result, our approach converts the parallelism plan space into a much smaller profiling space that scales with the structural diversity of the computation graph rather than the depth of the model.


Finally, we estimate the cost of each segment's parallelism plans using the profiling results and then use a \emph{dynamic programming} algorithm to optimize the plans of each segment, which can then be combined into a global intra-operator parallelism plan with the lowest total cost. 
We implemented the above analysis and optimization in the XLA compiler framework, leveraging its frontend and backend to build an automatic parallelization system, \sysname ({\em C}ommunication-{\em F}ree {\em P}reserve), for large model training. \sysname has been extensively evaluated across four models in various configurations on two target platforms. 
It outperforms state-of-the-art %automatic intra-operator parallel 
frameworks, TensorFlow-Alpa, achieving up to 1.51x, 1.31x, and 3.43x speedup on GPT, LLAMA, and MoE models, respectively. It optimizes parallelism plans for each model in less than 15 minutes.

==> CFP-VLDB-arxiv-v2/content/Limitation.tex <==
\vspace{-3mm}
\section{Conclusion}
%\section{Limitations and Discussion}

\sysname reduces the complexity of searching parallelism plans for large models by effectively exploiting the structural patterns of large models, thereby enabling an effective profiling-based method for accurate cost estimation and dynamic programming for plan optimization. While it has been proven to be effective in optimizing large model training plans, it has a couple of limitations that should be addressed in future work. First, \sysname does not consider additional levels of parallelism, such as pipeline parallelism. However, as discussed in Sec.\ref{scalability}, its segment sub-search space building and profiling method can be easily extended to pipeline parallel frameworks, providing more accurate stage profiles for pipeline stages partitioning. Second, \sysname does not account for multi-granularity overlapping between communication and computation, which increases uncertainty in downstream optimizations and widens the gap between symbolic cost and actual performance. We believe \sysname remains unaffected as it is based on runtime profiles.


% \textcolor{red}{(Rev-F: Adopting \sysname for inference)} (3) It has not been evaluated in inference scenarios. The key challenge is how to align the search for intra-operator parallel strategies with the optimization techniques widely used in inference. For example, compiler optimizations like operator fusion may conflict with the parallelization, and both of them are key optimizations to inference latency.

% \textcolor{red}{(Rev-E/F: Sensitivity of profiling data due to change in sparsity)} (4) \sysname's approach is inherently sensitive to dynamic sparsity, which is a common challenge for all compiler-based methods. however, we argue that \sysname can in fact reduce such affect: the profiling focuses on the boundaries of \pb, thus the potentially "noise" due to sparsity cannot accidentally affect the partition inside \pb.


==> CFP-VLDB-arxiv-v2/content/Method/ParallelBlock.tex <==

\section{ParallelBlock Construction}\label{chap3_label}

%\sysname constructs its core abstraction, \pb, by identifying parallelism-preserving subgraphs.  These \pb{}s are used as coarse-grained units to build the parallelism search space.
%and to split the model into model segments for profiling.

\subsection{Parallelism-preserving Subgraphs}\label{sec_pb_def}

Computation graphs inherently contain many subgraphs, such as chains of element-wise operators, which maintain the parallelism of input tensors throughout their computation.  
In these subgraphs, regardless of the dimension along which an input tensor is partitioned, the computation can proceed independently on each parallel partition from input to output.
We refer to such subgraphs as parallelism-preserving subgraphs.

Besides simple chains of element-wise operations, a parallelism-preserving subgraph may also include data manipulation and tensor contraction operators.
For example, in Fig. \ref{fig:parallelism-preserving_def}(a), an input tensor with shape \([A, B]\) is processed by a sequence of reshape and batched matrix multiplication (BMM) operators, producing an output tensor with the same shape.
The input tensor is first reshaped to a tensor of shape \([A, B_1, B_2]\), by splitting the second dimension of the original tensor into two dimensions of sizes \(B_1, B_2\), respectively, where \(B_1 \times B_2 = B\). 
This tensor is then multiplied with a parameter of size \([B_2, C, B_1]\) using BMM operator, contracting the dimension with size \(B_1\) and introducing a new dimension with size \(C\), resulting in an intermediate tensor of size \([B_2, A, C]\).  
Next, a second BMM with a parameter of shape \([B_2, B_1, C]\) further contracts the dimension with size \(C\) and restores the tensor to shape \([A, B_1, B_2]\).  
Finally, a reshape operation merges two dimensions with sizes \(B_1\), \(B_2\), producing an output tensor with same shape as input tensor.

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{content/Method/fig/parallelism_preserving_0701_v1.png}
    \vspace{-8mm}
    \caption{Parallelism-preserving examples. $B$, $S$, $H$, and $D$ in Self-Attention represent \textit{batchsize}, \textit{sequence length}, \textit{number of attention heads}, and the \textit{hidden size} of each head, respectively.  The computation graph is simplified for clarity.}
    \vspace{-4.5mm}
    \label{fig:parallelism-preserving_def}
\end{figure}


In this subgraph, the input tensor can be partitioned along the row dimension (size A), the column dimension (size B), or both.
Suppose the column dimension is mapped to an axis of the device mesh consisting of $P$ devices. 
We can observe that, if \(B_2\) is divisible by $P$, all tensor contractions in this subgraph can be performed independently within each parallel partition, without requiring inter-device communication.
Thus, the computation can proceed independently on each parallel partition from input to output.
This condition is commonly satisfied in practice, as intra-operator parallelism typically maps tensor dimensions to mesh axes with small power-of-two sizes (e.g., 2, 4, or 8), while tensor dimensions such as \(B_2\) are usually larger power-of-two (e.g., 16, 32, or 64).
% In this subgraph, as long as \(B_2\) is divisible by the parallelism degree (e.g., the number of GPUs), the computation can proceed independently on each parallel partition from input to output, regardless of whether the input tensor is parallelized along \(A\), \(B\), or both. 
% This means that the parallelism of each input tensor dimension can be "preserved" in the output tensor.

% A more complex example is the self-attention block in the Transformer, as illustrated in Fig. \ref{fig:parallelism-preserving_def}(b).
% Similarly, it can also be regarded as a parallelism-preserving subgraph as long as $B$ and $H$ are divisible by the number of devices along the corresponding mesh axis.
% This example provides a more intuitive way to illustrate the parallelism-preserving property: Fig.~\ref{fig:parallelism-preserving_def}(c) illustrated the element-level data dependency from its output tensor to its input tensors. 
% Each “block” of elements in the output tensor $Y$ depends only on the corresponding “blocks” of elements in the input tensors $Q$, $K$, and $V$. 
% That is, if the subgraph's computation is partitioned to multiple devices at the "block" granularity, the computation for each partition can be performed independently.

A more practical example is the self-attention block in the Transformer (Fig.~\ref{fig:parallelism-preserving_def}(b)), which provides a more intuitive illustration of the parallelism-preserving property.
Fig.~\ref{fig:parallelism-preserving_def}(c) illustrates the data dependency from its output tensor to its input tensors. 
Each “block” of elements in the output tensor $Y$ depends only on the corresponding “blocks” of elements in the input tensors $Q$, $K$, and $V$. 
That is, if the subgraph's computation is partitioned at the "block" granularity, the computation for each partition can be performed independently.
Similar to the subgraph in Fig.~\ref{fig:parallelism-preserving_def}(a), it can also be regarded as a parallelism-preserving subgraph as long as $B$ and $H$ are divisible by the number of devices along the corresponding mesh axis.


This parallelism-preserving property enables the construction of coarse-grained parallel units to reduce the intra-operator parallelism search space. 
However, identifying such subgraphs in the computation graph is highly challenging, as the computation graph only encodes tensor-level data dependencies. 
This makes it difficult to determine whether a subgraph’s output-to-input dependency stays within a parallel partition.  
As a result, prior work~\cite{zheng2022alpa, liu2023colossal} has relied on simple heuristics, such as merging operators based on their types.
However, such methods are insufficient to accurately identify parallelism-preserving subgraphs, especially those involving complex data manipulation and tensor contraction operators.


% Consider a tensor $Y$ with shape $[A_0, A_1, ..., A_{n-1}]$, where $A_i$ denotes the size, i.e., the number of elements, of the $i$-th dimension. 
% Each element of $Y$ is indexed as $Y(a_0, a_1, \dots, a_{n-1})$, where $a_i \in [0, A_i - 1]$ is an index along the $i$-th dimension.
% Similarly, for a tensor $X$ with shape $[B_0, B_1, ..., B_{m-1}]$, we can express the data dependency from an element in $Y$ to elements in $X$ using the following affine mapping:
% \begin{align}
% Y(a_0, a_1, \dots, a_{n-1}) \rightarrow X(b_0, b_1, \dots, b_{m-1}), \notag \\
% b_i = \sum_{j=0}^{n-1} k_{i,j} a_j + C_{i,j}, \quad 0 < i < m-1
% \end{align}
% \noindent
% The arrow indicates that the element in consumer tensor $Y$ \textit{depends on} the elements in producer tensor $X$.
% $k_j$ denotes the linear coefficient and $C_j$ denotes the constant offset for the $j$-th dimension.
% Each element in $Y$ is identified by an index tuple $(a_0, a_1, \dots, a_{n-1})$, and may depend on one or more elements in $X$.
% The index tuple $(b_0, b_1, \dots, b_{m-1})$ of each such element in $X$ is computed as an affine function of $(a_0, a_1, \dots, a_{n-1})$.

We address this challenge by modeling element-level data dependencies in the computation graph using affine transformation expressions, which enable the precise definition and identification of parallelism-preserving subgraphs.
Consider an output tensor $Y$ with shape $[A_0, A_1, ..., A_{n-1}]$, where $A_i$ denotes the size (the number of elements) of the $i$-th dimension. 
Each element of $Y$ is indexed as $\mathbf{a} = (a_0, a_1, \dots, a_{n-1})$, where $a_i \in [0, A_i - 1]$ is an index along the $i$-th dimension.
Similarly, for an input tensor $X$ with shape $[B_0, B_1, ..., B_{m-1}]$, we can express the data dependency from an element in $Y$ to elements in $X$ using affine mappings: 
$Y(\mathbf{a}) \rightarrow { X(\mathbf{b}) \mid \mathbf{b} \in \mathcal{F}(\mathbf{a}) }$.
where $\mathcal{F}(\mathbf{a}) = (f_0(\mathbf{a}), f_1(\mathbf{a}), ..., f_{m-1}(\mathbf{a}))$ specifies the set of input indices that $Y(\mathbf{a})$ depends on.
Each $f_k(\mathbf{a})$ is an affine function of $\mathbf{a}$ that may return either a single integer (a scalar index) or a set of integers (a set of element indices) along the $k$-th dimension of $X$.


\begin{table}[t]
  \centering
  \caption{Affine mappings for different type of operators. 
  The dimension specification indicates how tensor indices change based on the semantics of the operator. 
  }
  \vspace{-2mm}
  \adjustbox{max width=\linewidth}{
  \begin{tabular}{ccc}
    \toprule
    Type of Op & Dimension Specifications & Affine Mappings \\
    \midrule
    Elem-wise & / & $f_i(\mathbf{a}) = a_i$ \\
    Reshape & Split dimension $k$ to $k, k+1$ & 
    $\begin{cases}
      f_i(\mathbf{a}) = a_i & i < k \\
      f_k(\mathbf{a}) = K_{a+1} a_k + a_{k+1} \\
      f_i(\mathbf{a}) = a_{i+1} & i > k
    \end{cases}$ \\
    Reshape & Merge dimensions $k, k+1$ to $k$ & 
    $\begin{cases}
      f_i(\mathbf{a}) = a_i & i < k \\
      f_k(\mathbf{a}) = \left\lfloor a_k / B_{k+1} \right\rfloor \\
      f_{k+1}(\mathbf{a}) = a_k \bmod B_{k+1} \\
      f_i(\mathbf{a}) = a_{i-1} & i > k+1
    \end{cases}$ \\
    Transpose & Permute dimensions $i \rightarrow \pi(i)$ & 
    $f_i(\mathbf{a}) = a_{\pi(i)}$ \\
    Broadcast & Add dimension $k$ & 
    $\begin{cases}
      f_i(\mathbf{a}) = a_i & i < k \\
      f_i(\mathbf{a}) = a_{i-1} & i \geq k
    \end{cases}$ \\
    Contraction & Reduce dimension $k$ & 
    $\begin{cases}
      f_i(\mathbf{a}) = a_i & i \ne k \\
      f_k(\mathbf{a}) = \{ c \mid 0 \leq c < B_k \} \\
    \end{cases}$ \\
    \bottomrule
  \end{tabular}
  }
  \label{tab:deps_for_op}
  \vspace{-3.5mm}
\end{table}

Taking the dependency from a single operator's output tensor to its input tensor as examples, as shown in Table~\ref{tab:deps_for_op}. 
For a simple element-wise operator, each output element depends on the input element with the same index, i.e., $m=n$, and $f_i(a_0, ..., a_{n-1}) = a_i$, for $0 \leq i<n$.
For a reshape operator that splits the $k$-th dimension of the input tensor into two consecutive dimensions, the $k$-th and the $k+1$-th, in the output tensor.
If the original input dimension of size $B_k$ is split into two output dimensions of sizes $A_k$ and $A_{k+1}$, where $A_k A_{k+1}=B_k$.
Then each output element indexed by $\mathbf{a} = (a_0, \dots, a_{n-1})$ depends on the input element indexed by $\mathcal{F}(\mathbf{a}) = (f_0(\mathbf{a}), \dots, f_{m-1}(\mathbf{a}))$,
where:
(1) $f_i(\mathbf{a}) = a_i$ for $i < k$,
(2) $f_k(\mathbf{a}) = A_{k+1} a_k + a_{k+1}$, and
(3) $f_i(\mathbf{a}) = a_{i+1}$ for $i > k$.
That is, the dependent element's index along the $k$-th dimension is computed by combining indices of two split dimensions, while the indices for other input dimensions are either copied directly (for $i < k$) or taken from the corresponding shifted positions in the output (for $i > k$) due to the insertion of a new dimension.


We further characterize the property that the computation of each parallel partition can proceed independently without requiring elements from other partitions.
% \sout{
% This property is reflected in the element-level dependency between the subgraph's input and output tensors, where the dependent input elements of each output element must lie entirely within the same parallel partition of the input tensor.
% Based on this, we define the formal condition for identifying parallelism-preserving subgraphs.
% }
A subgraph can be regarded as a parallelism-preserving subgraph if there exists a set of positive integers $d_0, d_1, ..., d_{n-1}$, such that, for $0 \le i < n$, the affine mappings between any input tensor $X$ and any output tensor $Y$ satisfy:
\begin{align}
    f_{i}(\mathbf{a}) = \lfloor \frac{a_i}{d_i} \rfloor d_i + c: 
     \quad 0 \leq c<d_i, \quad \frac{A_i}{d_i}  \bmod  P_i = 0\label{eq:stop_grouping_criteria}
\end{align}
\noindent
where $P_i$ represents the number of devices along the device mesh axis to which the $i$-th tensor dimension is mapped.
This indicates that the input and output tensors of a parallelism-preserving subgraph have the same tensor dimensions, and the  dependency in each dimension remains within the corresponding parallel partition. 

% \sout{
% For example, the element-level data dependency from output tensor $Y$ to input tensor $V$ in Fig.\ref{fig:parallelism-preserving_def} is 
% }
% \begin{equation}
% Y(i_0,i_1) \rightarrow V(\lfloor \frac{i_0}{S} \rfloor S + s, i_1) : { 0 \leq s<S}, \frac{A_0}{S} = B
% \label{dep_y_to_v}
% \end{equation}
% \noindent
% \sout{
% where $A_0 = B*S$ is the first dimension size of tensor $V$, $S$ is the sequence length in Transformer models, and $B$ is batchsize for training. 
% In practice, the batchsize is usually divisible by the number of devices for intra-operator parallel training.
% }

% \begin{table}[t]
%   \centering
%   \caption{Affine expressions for different types of operators. The dimension specification indicates how tensor indices change based on the semantics of the operator. K represents the interval for splitting a tensor dimension in Reshape operations, and ``*'' denotes any element along a tensor dimension. Tensor prefixes and irrelevant dimensions are omitted for clarity.}
%   \vspace{-2mm}
%   \adjustbox{max width=\linewidth}{
%   \begin{tabular}{ccc}
%     \toprule
%     Type of Op & Dimension Specifications & Affine Expression \\
%     \midrule
%     % Elem-wise & / & $(a_0, a_1, ..., a_n)\rightarrow(a_0, a_1, ..., a_n)$ \\
%     Elem-wise & / & $(..., a_i, ...)\rightarrow(..., b_i, ...), b_i=a_i$ \\
%     Reshape & Split dimension $i$ to $i, i+1$ & $(..., a_i, a_{i+1}, ...)\rightarrow(.., b_i, ...), b_i=Ka_i+a_{i+1}$ \\
%     Reshape & Merge dimensions $i, i+1$ to $i$ & $(..., a_k, ...) \rightarrow (..., b_i, b_{i+1}, ...),\ b_i = \lfloor a_k / K \rfloor,\ b_{i+1} = a_k \% K$ \\
%     Transpose & Target dimensions: $i_0, i_1, ..., i_n$ & $(a_0, a_1, ..., a_{n-1})\rightarrow(b_0, b_1, ..., b_{n-1}),\ b_j = a_{i_j}$ \\
%     Broadcast & Add dimension $i$ & $(..., a_i, ..., ) \rightarrow (..., b_i, ...),\ b_j = a_j \text{ for } j < i,\ b_j = a_{j+1} \text{ for } j \ge i$ \\
%     Contraction & Contraction dimension $i$ & $(..., a_i, ...) \rightarrow (..., b_i, ...), a_j = b_j \text{for } j < i, a_j = b_{j+1} \text{for } j \ge i$ \\
%     \bottomrule
%   \end{tabular}
%   }
%   \label{tab:deps_for_op}
% \end{table}

% \begin{table}[t]
%   \centering
%   \caption{Affine mappings for different type of operators. 
%   The dimension specification indicates how tensor indices change based on the semantics of the operator. 
%   % K represents the interval for splitting a tensor dimension in Reshape operations.
%   \textcolor{blue}{Affine functions for irrelevant dimensions are omitted for clarity}.
%   }
%   \vspace{-2mm}
%   \adjustbox{max width=\linewidth}{
%   \begin{tabular}{ccc}
%     \toprule
%     Type of Op & Dimension Specifications & Affine Mappings \\
%     \midrule
%     Elem-wise & / & $f_i(\mathbf{a}) = a_i$ \\
%     Reshape & Split dimension $k$ to $k, k+1$ & 
%       $f_k(\mathbf{a}) = A_{k+1} a_k + a_{k+1}$ \\
%     Reshape & Merge dimensions $k, k+1$ to $k$ & 
%     $\begin{cases}
%       f_k(\mathbf{a}) = \left\lfloor a_k / B_{k+1} \right\rfloor \\
%       f_{k+1}(\mathbf{a}) = a_k \bmod B_{k+1} \\
%     \end{cases}$ \\
%     Transpose & Permute dimensions $i \rightarrow \pi(i)$ & 
%     $f_i(\mathbf{a}) = a_{\pi(i)}$ \\
%     Broadcast & Add dimension $k$ & 
%     $\begin{cases}
%       f_i(\mathbf{a}) = a_i & i < k \\
%       f_i(\mathbf{a}) = a_{i-1} & i \geq k
%     \end{cases}$ \\
%     Contraction & Reduce dimension $k$ & $
%       f_k(\mathbf{a}) = \{ c \mid 0 \leq c < B_k \}$ \\
%     \bottomrule
%   \end{tabular}
%   }
%   \label{tab:deps_for_op}
% \end{table}

For a path in the computation graph, \sysname incrementally builds affine mappings for each operator along the path and composes them.
% To construct element-level dependencies between tensors in the computation graph, \sysname incrementally builds affine transformations for operators along the dependency path and composes them.
It starts by assigning identity affine mappings to a given input tensor. 
Then, for each subsequent operator, it builds specific affine mappings based on operator's type and dimension specification, as shown in Table.\ref{tab:deps_for_op}.
These affine mappings are composed with the accumulated mapping from previous operators. 
Through this recursive composition, \sysname maintains an up-to-date mapping relation that describes how each element of the current tensor depends on the original input tensor.
% For each operator, \sysname constructs its transformation affine expression based on its type and dimension specification, as shown in Table.\ref{tab:deps_for_op}.
% \sout{
% For example, the data dependency from tensor $Y$ to tensor $V$ in Eq.\ref{dep_y_to_v} is derived by composing the affine expressions of the three operators along their dependency path:
% }
% \begin{equation}
% I_R(i_0, i_1, i_2, i_3) \rightarrow V(Si_{0}+i_{2}, Di_{1}+i_{3})
% \end{equation}
% \begin{equation}
% I_M(i_0, i_1, i_2, i_3) \rightarrow I_R(i_0, i_1, *, i_3)
% \end{equation}
% \begin{equation}
% Y(i_0, i_1) \rightarrow I_M(\lfloor i_{0}/{S}\rfloor, \lfloor i_{1}/{D}\rfloor, i_{0}\%S,  i_{1}\%D)
% \end{equation}
% \noindent
% \sout{
% where $I_R$ is the intermediate tensor obtained by applying reshape operator to tensor $V$, $I_M$ is the intermediate tensor obtained by further applying BMM operator to $I_R$.
% }




% 最初的逻辑：
% 1.定义parallelblock是算子+子图，性质是保持一致并行维度
% 2.说明合理性：
% - 分析什么情况下最优，什么情况下不是最优
% - 介绍什么是cheaper resharding(子图中存在可以作为resharding位置的中间张量)，当存在cheaper resharding时切分ParallelBlock，切分后的ParallelBlock能保持最优。
% 3. PB的构造，group子图，检测到cheaper resharding时切分PB

% 写theorem就需要在给出theorem时附加前提条件：ParallelBlock包含的不是算子+任意子图，而是没有cheaper resharding的子图。

% 可选的逻辑1
% 不定义“没有cheaper resharding的子图”，维持原本的ParalleBlock定义，在构造过程说明ParalellBlock对potential resharding的检测与切分过程。这时theorem只针对所构造出的这类ParallelBlock.
% 1. ParallelBlock definition: 一个算子+子图，性质…
% 2. 构造过程：grouping process 
% 3. post-group checking “cheaper resharding” and spliting PB，说明什么是“cheaper resharding”,为什么要这样做checking 和 spliting。
% 4. theorem: parallelblock的这种“构造”是最优的，不会排除全局最优并行方案。
% 5. proof sketch： 当前后parallel diemsion一样时，内部的resharding是冗余的。当前后parallel dimension不一样时，resharding可以推迟到子图输出。

% 可选的逻辑2
% 直接定义没有cheaper resharding的子图，再定义ParallelBlock (3.1概念很多，这里直接引入新概念不太好）
% 1. 当子图中所有可用于tensor resharding的中间结果张量的大小不小于输出张量时，是一个没有cheaper resharding的子图
% 2. ParallelBlock definition: 一个算子+没有cheaper resharding的子图，性质…
% 3. theorem: parallelblock的这种“定义”是最优的，不会排除全局最优并行方案。
% 4. proof sketch：...
% 5. 构造过程：grouping process + post-group checking and spliting PB.


% 可选的逻辑3
% 构造过程引出对"cheaper resharding 子图"的定义，之后再定义ParallelBlock。（感觉比较合理）
% 动机(简化搜索空间)引出构造过程→gourping process→post-group check:说明“cheaper resharding”的概念→定义ParallelBlock(operator+cheaper resharding free subgraph)→theorem and proof:
% 1. 承接上文对parallelism-preserving subgraph的介绍，说明在直觉上，我们可以在计算图上定位这些子图，并利用这种并行保留的性质，将他们合并成大的并行单元
% 2. 构造过程：grouping process 
% 3. post-group checking “cheaper resharding” and spliting PB，说明什么是“cheaper resharding”,为什么要这样做checking 和 spliting。
% 4. 定义：ParallelBlock是一个算子+no cheaper resharding的子图，性质:xxxx
% 5. theorem: parallelblock的这种“定义”是最优的，不会排除全局最优并行方案。
% 6. proof sketch：...

\vspace{-2mm}
\subsection{ParallelBlocks}\label{sec_group_op}

Intuitively, we can group operators in such subgraphs and apply consistent parallel dimensions throughout. 
This allows us to eliminate the need to exhaustively combine strategies for individual operators by pruning away suboptimal combinations. 
Motivated by this, \sysname constructs coarse-grained structures, \pb{}s, which serve as basic parallel units for intra-operator parallelization.
The construction of \pb{}s proceeds in two phases:

\textbf{Phase 1: Operator grouping}.
Since tensor contraction operators are more likely to cause dimension reductions or expansions that disrupt the parallelism-preserving property, \sysname treats each of them as a starting point for dependency analysis to incrementally identify the downstream parallelism-preserving subgraph.
Each tensor contraction operator is then grouped with all downstream operators within this subgraph.

The grouping process is illustrated in Algorithm \ref{BuildPB}.
Tensor contraction operators are first sorted by their depth in the computation graph.
For each one, \textit{DFSAndGroup} explores the downstream operators in a depth-first manner and groups those that belong to the same parallelism-preserving subgraph.
At each step, it checks the data dependency relationship using the condition stated in Eq.~\ref{eq:stop_grouping_criteria}.

%it checks whether the data dependency from the current operator’s output tensor to the tensor contraction output tensor satisfies the condition in Eq.~\ref{eq:stop_grouping_criteria}.

% For each tensor contraction operator, \textit{DFSAndGroup} starts from its output tensors to find the flowing parallelism-preserving subgraph and groups them with the tensor contraction operator.
% The \textit{DFSAndGroup} function checks whether the output tensor of each user (i.e., the operator that consumes the current operator’s output tensor) satisfies the data dependency criteria outlined in Eq.~\ref{eq:stop_grouping_criteria}, and recursively traverses each user’s own users on the DFG (\textit{GetAllUsers()}) in a depth-first manner.
% The traversal process terminates when there are no subsequent operators, or when the data dependencies along the traversal path do not satisfy the parallelism-preserving conditions.

\textbf{Phase 2: Refinement}.
%After the grouping process, \sysname performs a post-grouping refinement to identify \textit{parallelism-preserving subgraph with internal resharding opportunities}.
% Operators in a parallelism-preserving subgraph may temporarily reduce or expand the size of intermediate tensors.
% When the size is reduced, the resulting smaller intermediate tensors have the potential to serve as cheaper resharding points in certain globally optimal parallelism plans. 
% Specifically, if a globally optimal plan assigns incompatible parallel dimensions to the operators before and after the subgraph, a resharding must be inserted between them.
% In this case, the globally optimal plan may therefore choose to reshard the smaller intermediate tensor to bridge the inconsistency in parallel dimensions.
% As a result, grouping such parallelism-preserving subgraph with its preceding operator with strict parallel dimension consistency can obscure the cheaper resharding opportunities.
Assume a globally optimal parallelism plan assigns inconsistent parallel dimensions to two operators located before and after a parallelism-preserving subgraph, respectively.
In this case, a tensor resharding is required somewhere between these two operators. 
%to bridge the mismatched parallel dimensions.
The optimal plan may prefer to choose the smallest intermediate tensor produced between the two operators for resharding to minimize communication overhead.
If such a tensor is part of the parallelism-preserving subgraph, treating this subgraph as a unit for parallelization may hinder internal resharding opportunities.
More specifically, there are two typical patterns that can lead to such internal resharding opportunities: (1) Multiple tensor contractions, where an input tensor dimension is first split into two dimensions, one of which is contracted and later projected back to the original shape. (2) Complex data manipulation operators (slicing or gather operations with certain patterns) that extract subsets or supersets of the input tensor and are later broadcast or reduced to match the expected output.

\setlength{\textfloatsep}{5pt}
\begin{algorithm}[t]
\small
\caption{DFS for Constructing ParallelBlock. }
\label{BuildPB}
\Input{ Computation Graph $G$}
\Output{ ParallelBlocks $PBS$: Lists of operators }
\SetKwFunction{MainFunc}{BuildParallelBlocks}
\SetKwFunction{SubFunc}{DFSAndGroup}
\SetKwFunction{SortTensorContractionOpSet}{SortTensorContractionOpSet}
\SetKwFunction{IsGrouped}{IsGrouped}
\SetKwFunction{SetGrouped}{SetGrouped}
\SetKwFunction{GetAllUsers}{GetAllUsers}
\SetKwFunction{AddOtherOperandToPB}{AddOtherOperandToPB}
\SetKwProg{Fn}{Function}{:}{\KwRet} 
\Fn{\MainFunc{$G$}}{
$PBS$ = \{\} \;
$S$ = \SortTensorContractionOpSet{$G$}\;
\For{each $s$ in $S$}{
    $PB$ = \{\} \;
    \If{\IsGrouped{$s$}}{
        continue\;
    }
    \Else{
        Add $s$ to $PB$\;
        \SubFunc{$s, PB$}\;
        \SetGrouped{$PB$}\;
    }
    Add $PB$ to $PBS$\;
}
\KwRet{$PBS$}\;
}
\Fn{\SubFunc{$op, PB$}}{
$users$ = {\GetAllUsers{$op$}}\;

\For{each $user$ in $users$}{
        \If{\IsGrouped{$user$}}{continue\;}
        \Else{
            \If{Check $user, PB$ with Eq.(\ref{eq:stop_grouping_criteria})}{
                Add $user$ to $PB$\;
                %\tcp*{Add other operands of user to PB.}
                % \AddOtherOperandToPB{$user, PB$}\;
                \KwRet{\SubFunc{$user, PB$}}\;
            }

        }
}
\KwRet{}\;
}
\end{algorithm}

Based on this, 
\sysname identifies
each parallelism-preserving subgraph that contains multiple tensor contractions or complex data manipulation operators, where an intermediate tensor is smaller than the subgraph’s output. \sysname then splits it at the corresponding resharding point, yielding two separate subgraphs.

\textbf{\pb}.
We define each subgraph constructed through the two-phase process as a \pb{}.
A \pb is a subgraph within which no internal resharding opportunity exists.
The parallel dimensions of operators in the \pb are determined by those of its first operator. %This constraint ensures that the candidate parallelism strategies of the \pb{} are fully determined by the strategies of its first operator,  rather than the combination of strategies from all operators within it.

\begin{theorem}
% A \pb forms a closure under intra-operator parallelization: 
Enforcing consistent parallel dimensions throughout a \pb does not exclude the globally optimal parallelism plan from the reduced search space.
\end{theorem}

\textbf{Proof sketch.}
Consider a parallelism-preserving subgraph in the computation graph and a globally optimal parallelization plan.
There are two cases:

\textbf{Case 1:} The optimal plan assigns \emph{consistent} parallel dimensions to the operators located immediately before and after the subgraph. In this case, using parallel dimensions consistent with those of the preceding operator throughout the whole subgraph is necessary. Otherwise, it would introduce additional tensor resharding within the subgraph, which cannot be part of the optimal plan.

\textbf{Case 2:} The optimal plan assigns \emph{inconsistent} parallel dimensions to the operators located immediately before and after the subgraph.
In this case, tensor resharding is inevitable.
Since the parallelism-preserving subgraph in \pb is refined to exclude potential internal resharding opportunities, performing the resharding on the subgraph’s output tensor would not introduce additional communication overhead in comparison to resharding any intermediate tensors within the subgraph.

In both cases, enforcing consistent parallel dimensions throughout a \pb does not exclude the globally optimal parallelization plan.$\square$


\textbf{Construction complexity.}
Given a computation graph contains $N$ operators and $E$ edges. Let $T$ be the number of tensor contraction operators, and $K$ be the number of \pb{}s requiring intermediate tensor checks ($K < T$). Assume each such \pb{} contains on average $L$ edges.
The construction involves three steps:
(1) Sorting the $T$ contraction operators based on topological depth, which requires $O(N + E + T \log T)$ time.
(2) Constructing each \pb using DFS traversal, taking $O(N + E)$ as each operator and edge is visited at most once, to construct the affine transformation and compose it with previous accumulated dependency;
(3) For $K$ \pb{}s, checking edges (intermediate tensors) to find potential cheaper resharding points, with $O(K \cdot L)$ complexity.
Overall, the total time complexity is $O(N + E + T \log T + K \cdot L)$, which approaches $O(N + E)$ in practice since $T \ll N$ and $K \cdot L < E$.

\vspace{-1mm}
\subsection{Parallelism Plan Construction}\label{SearchSpace}                                     
To generate an intra-operator parallelism plan for computation graph, each operator should be assigned a parallelism strategy. 
\sysname first selects a parallelism strategy for the first operator of each \pb, and then automatically infers the parallelism strategies for all operators in the computation graph.

As shown in Fig.\ref{fig:parallel_plan}(a) to \ref{fig:parallel_plan}(b), the parallelism strategies of the operators within the two {\pb}s can be inferred by propagating the parallel dimensions of the first operator.
Operators in model parameter input branches are not grouped into {\pb}s because they lie outside the traversal path in \pb construction process. 
\sysname finds the operator within the \pb that receives this input branch and propagates its parallel dimensions back to the input branch. 
In Fig.\ref{fig:parallel_plan}(b), the parallel dimensions of the right side parameter are determined based on the parallel dimensions of operators in the second \pb.

In addition, some operators may generate tensors used by multiple {\pb}s, and the parallel dimension requirements of different {\pb}s for these operators may conflict. 
% This makes their parallelism strategies cannot be easily inferred from a single {\pb}.
\sysname identifies the data dependency paths from these operators to all related {\pb}s and determines compatible parallelism strategies for them, as shown in Fig. \ref{fig:parallel_plan}(c).

Based on the parallelism plan construction process, \sysname builds the intra-operator parallelism search space by combining the parallelism strategies of all {\pb}s on computation graph, and then constructs a parallelism plan for each instance within the space.
The intra-operator parallelism search space is reduced to a combination of parallelism strategies for a few key operators instead of all operators, 
i.e., for a part of the model with $N$ {\pb}s and $D_i$ parallelism strategies for the i-th \pb, 
the size of the parallelism search space is $S = \prod_{i=1}^{N} D_i$.



==> CFP-VLDB-arxiv-v2/content/Method/Profile.tex <==

\section{Profiling Model Segments}\label{chap4_label}

%可以删掉
% By constructing a coarser-grained parallel unit, \pb, we create an intra-operator parallelism search space that depends on the number of {\pb}s and the parallelism strategies of each \pb. 
% However, directly applying profiling to evaluate the cost of every instance in this space will still results in significant profiling overhead, making it impractical to complete within a reasonable time.
% As the number of model layers increases, there will still be a considerable number of {\pb}s, leading to a expansion of the parallelism search space. Additionally, since profiling requires multiple runs of the parallel program, the increased model depth also results in longer run times for every profiling step, further increasing the profiling overhead.

% Based on the computation graph compression achieved by \pb{}s, 
%\sysname leverages repetitive patterns in model structure to extract a set of distinct segments, profiles them separately, and combines the profiles to get the cost of a global parallelism plan. 

% \subsection{Segment Generation}

% \sysname identifies repeated computational patterns in the model by segmenting the computation graph into a small number of distinct segments. 
% Each segment shares the same parallelism search space and exhibits similar parallel execution behavior, allowing its physical execution cost to be profiled once and reused across all instances.
%可以删掉
% A straightforward approach is to rely on user-defined annotations at the compiler front-end to specify which repeated model structures should be recognized as unique segments.
% However, this not only demands manual effort from model developers with performance tuning experience, but also suffers from inconsistency: such layer definitions may not compile into identical dataflow graphs.
% Variations in data dependencies can prevent them from achieving the same communication behaviors under the same parallelism plans.
% Another approach approach is to directly search for identical dataflow subgraphs in the computation graph. 
% However, this method not only incurs significant search overhead but may fail to match segments with the same parallel behavior, due to minor differences in trivial operators such as data reorganizations.
%
% Thanks to the {\pb}-based modeling of computation graph, the graph can be represented as a sequence of {\pb}s in terms of intra-operator parallelization.
% Any two model segments must have aligned \pb sequences to have the same parallelism search space and similar parallel execution behavior.
% We thus transforms the extraction of distinct segments into a pattern matching problem on the sequence of {\pb}s. 
% That is, the comparison granularity 
%
% This segmentation is achievable due to the graph's representation based on \pb. 
% Instead of matching arbitrary operator-level subgraphs, \sysname uses \pb{}s as the matching granularity, turning segment identification into a sequence matching problem over \pb{}s.
% Instead of matching arbitrary operator-level subgraphs, \sysname models the graph as a linear sequence of \pb{}s, each capturing a coarse-grained parallel unit.
% Consequently, segment identification becomes a subsequence matching problem over the \pb sequence.



%huwf0429 简化篇幅
% Comparing \pb sequences is still challenging because it is essentially a computation subgraph with fine-grained operators. 
% Moreover, even if two \pb sequences contain the same set of operators, they may not exhibit similar parallel execution behavior under same plans due to differences in data dependencies.
% To address this, \sysname extracts fine-grained data dependency graphs of tensor contraction operators from \pb subsequence, using them as fingerprints for sequence matching.

% For subsequence matching, \sysname extracts fine-grained data dependency graphs of tensor contraction operators from \pb subsequences and uses them as fingerprints.
% Matching tensor contraction operators ensures that the compared subsequences share the same parallelism search space, while further aligning the fine-grained data dependencies between these tensor contraction operators guarantees the consistent parallel execution behavior (e.g., identical communication patterns) under same plans.

% However, directly comparing all operators within \pb{} sequences is impractical for two main reasons. First, each \pb{} typically contains a large number of operators, making exhaustive operator-level comparison computationally expensive. 
% Second, strict matching at the operator level can lead to mismatches between semantically equivalent segments due to trivial variations. 
% For example, one model layer may explicitly reshape a parameter tensor before use, while another functionally identical layer may consume the same tensor directly without reshaping. 
% Such discrepancies do not affect the semantics or parallel execution behavior of the segment but can disrupt matching.

% To address this, \sysname extracts key structural features, referred to as fingerprints, from each \pb subsequence to serve as the basis for comparison.
% These fingerprints are derived from the data dependency graphs of tensor contraction operators within a \pb sequence, where each dependency edge is annotated with element-level affine mappings.
% Matching tensor contraction operators ensures that the segments share the same parallelism search space and similar computation workload, as other operator types typically incur negligible computation overhead.

% Further aligning the element-level data dependencies ensures consistent tensor layouts and resharding operations,
% which in turn leads to identical communication patterns under the same parallel plans.
% Fig.\ref{fig:model_segment} shows a simple \pb sequence containing three subsequences, each with two {\pb}s. 
% The element-level data dependency graph of tensor contraction operators in each subsequence is extracted to serve as a fingerprint for comparison. 
% The first two subsequences do not match because, despite having the same operators within the {\pb}s, differences in dependencies between tensor contraction operators cause inconsistent communication patterns when both subsequences are assigned same parallelism plans. 
% For example, 
% keeping the same parallel dimension between two \pb{}s inside them. 
% In the first subsequence, a communication is required between the two \pb{}s to resharding intermediate results, whereas the second require no communication.
% However, the last two subsequences share the same fingerprints, ensuring that they have consistent parallelism search space and similar execution behavior under same plans, despite minor difference in other type operators.
% Note the fingerprinting-based matching does not require the data flow graphs of segments to be exactly the same. 
% This is because the fingerprint ensures the consistency of tensor contraction operators between segments, while the computational overhead of other types of operators is negligible.

% Fig.\ref{fig:model_segment} shows a simple \pb sequence containing three subsequences, each with two {\pb}s. 
% % As illustrated in Fig.\ref{fig:model_segment}, each subsequence consists of two \pb{}s.
% Although the first and second subsequences contain the same tensor contraction operators, they differ in how intermediate results are consumed.
% As a result, such differences in data dependencies may lead to divergent communication patterns under identical parallelism plans, for example, one subsequence may require additional resharding of intermediate results while the other does not.
% In contrast, despite minor differences in non-tensor contraction operators, the last two subsequences have identical fingerprints, thus exhibit similar execution behavior under same plans.

% \sysname uses a simple greedy search algorithm to find a set of subsequences that can cover the original {\pb} sequence, while keep the number of distinct subsequences as low as possible.
% \sysname leverages the fingerprint mechanism to perform template matching over the \pb{} sequence, aiming to identify a minimal set of representative subsequences that collectively cover the entire model. 
% It builds a match table by comparing fingerprints of all candidate subsequences and employs a dynamic programming algorithm to select the smallest set of segments with full coverage. 
% This approach enables efficient identification of repetitive patterns in model structure.



\subsection{Segment Generation}
\sysname identifies repeated computational patterns in the model by extracting a small number of distinct segments from the computation graph. 
Each type of segment shares the same parallelism search space and exhibits similar parallel execution behavior, allowing its physical execution cost to be profiled once and reused across all instances.
This extraction is achievable due to the graph's representation based on \pb. 
Instead of matching arbitrary operator-level subgraphs, \sysname uses \pb{}s as the matching granularity, turning segment identification into a sequence matching problem over \pb{}s.

However, directly comparing all operators within \pb{} sequences is impractical for two main reasons. First, each \pb{} typically contains a large number of operators, making exhaustive operator-level comparison computationally expensive. 
Second, strict matching at the operator level can lead to mismatches between semantically equivalent segments due to trivial variations. 
For example, one model layer may explicitly reshape a parameter tensor before use, while another functionally identical layer may consume the same tensor directly without reshaping. 
Such discrepancies do not affect the semantics or parallel execution behavior of the segment but can disrupt matching.

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{content/Method/fig/parallel_dimension_inference.png}
    \vspace{-3mm}
    \caption{Inferring parallelism plan for a given parallelism strategy for each \pb.}
    \label{fig:parallel_plan}
\end{figure}


To address this, \sysname first searches for pairs of \pb{} subsequences that have the same key operators (i.e., the first operator in each \pb).
Since these operators dominate the choice of parallelism strategies of the subsequence, matching them ensures that the subsequences share the same parallelism search space.
To further determine whether these subsequences exhibit similar physical execution behaviors, \sysname extracts the data dependency graphs of tensor contraction operators from each subsequence as \textit{fingerprints} for comparison.
%Each fingerprint is constructed as a data dependency graph extracted from the tensor contraction operators within a \pb{} subsequence.
In this data dependency graph, each node represents a tensor contraction operator, and each edge is annotated with an element-level affine mapping that encodes how the output elements of one tensor contraction operator are consumed by another.
The construction of these affine mappings follows a similar process in Section~\ref{chap3_label}, i.e., composing the affine mappings of each operator along the dependency path.

\sysname then leverages this matching mechanism to perform template matching over the \pb{} sequence, aiming to identify a minimal set of representative subsequences that collectively cover the entire model. It builds a match table by comparing the fingerprints of all candidate subsequences and employs a dynamic programming algorithm to select the smallest set of segments with full coverage.


The rationale of the design of fingerprints is twofold.
\textbf{Ensuring similar execution behaviors.}
Tensor contraction operators typically dominate the computational cost, while other operator types incur negligible overhead.
Therefore, matching contraction patterns guarantees similar computation workloads.
In addition, aligning the element-level data dependencies among tensor contraction operators ensures that the same parallel strategy produces consistent intermediate tensor layouts and resharding behaviors, resulting in identical communication patterns.

\textbf{Improving matching efficiency.}
Fingerprint-based comparison not only avoids the high cost of exhaustive operator-level matching but also abstracts away trivial variations, such as explicit reshaping, that would disrupt matching.


Fig.\ref{fig:model_segment} shows a simple \pb sequence containing three subsequences, each with two {\pb}s. 
% As illustrated in Fig.\ref{fig:model_segment}, each subsequence consists of two \pb{}s.
Although the first and second subsequences contain the same tensor contraction operators, they differ in how intermediate results are consumed.
As a result, such differences in data dependencies may lead to divergent communication patterns under identical parallelism plans. For example, one subsequence may require additional resharding of intermediate results while the other does not.
In contrast, despite minor differences in non-tensor contraction operators, the last two subsequences have identical fingerprints, thus exhibit similar execution behavior under the same plans.

\begin{figure}
    \centering
    \includegraphics[width=0.40\textwidth]{content/Method/fig/fingerprint_0623.png}
    \vspace{-4mm}
    \caption{Identify distinct model segments based on \pb subsequences using element-level dependency graph of tensor contraction operators within \pb{}s.}
    \label{fig:model_segment}
    \vspace{-1mm}
\end{figure}

\vspace{-2mm}
\subsection{Profiling Mechanism}\label{profling_method}

\sysname first combines all {\pb}s' strategies to construct a sub-search space for each distinct segment.
It then profiles the communication and computation overhead for each parallelism plan in the sub-search space.
Profiling communication overhead is essential as it varies significantly across different plans.
Computation overhead is also profiled because different ways of partitioning operators can affect device utilization of computation kernels.
% Computation overhead is profiled for two reasons:
% (1) different communication patterns can lead to extra data movement, such as data splitting and concatenation; and 
% (2) different ways of partitioning operators can affect compilation, memory optimization, and \textcolor{black}{device utilization of computation kernels in accelerate libraries such as CUBLAS.}


Directly aggregating the profiled results of all segments does not fully capture the cost of a global parallelism plan, because cross-segment tensor dependencies may introduce additional resharding overhead when the connected segments adopt incompatible strategies.
A straightforward solution is to enumerate all connected distinct segment pairs and profile the resharding overhead under every combination of their parallelism plans. 
However, this leads to a combinatorial explosion, as the number of combinations grows exponentially with the number of distinct segments and plans.


\sysname identifies cross-segment tensor dependencies in the computation graph and locates the corresponding source and destination \pb{}s involved in each dependency.
It then profiles the resharding overhead for these \pb{} pairs under all combinations of their parallel strategies.
This significantly reduces the profiling space while still capturing the cross-segment resharding cost needed for accurate modeling.
% Cross-segment dependencies usually only involve the input tensor of the second segment and the output tensor of the first segment. 
% Therefore, the profiling overhead for tensor resharding overhead between segments is much lower than that for individual segments.
In practice, most cross-segment dependencies occur at segment boundaries, where the output tensor of one segment is directly consumed as the input tensor of the next.
Therefore, the profiling space for cross-segment tensor resharding is much lower than that for individual segments.

% Overall, \sysname leverages the compiler backend to generate SPMD programs for all parallelism plans of each distinct segment, as well as for all cross-segment resharding cases. It then runs these programs multiple times to collect two types of profiles for all distinct segments:
% (1) communication kernel time $c$, computational kernel time $p$, and peak memory consumption $m$ under different parallelism plans;
% (2) communication kernel time $r$ for tensor resharding between connected cross-segment \pb pairs.

Overall, \sysname leverages the compiler backend to generate SPMD programs for all parallelism plans of each distinct segment, as well as for all cross-segment resharding cases. It then runs these programs multiple times to collect two types of profiles for all distinct segments:
(1) communication kernel time, computational kernel time, and peak memory consumption under different parallelism plans;
(2) communication kernel time for tensor resharding between connected cross-segment \pb pairs.

\vspace{-2mm}
\subsection{Profiling Overhead Analysis}

% 可以删掉
% The complexity of the proposed profiling method depends on the number of distinct repeated structural patterns and the coverage of parallelism-preserving subgraphs within each segment.
Assume that a model has $M$ {\pb}s and $N$ distinct segments, the $i$-th distinct segment contains $K_i$ {\pb}s, and the $j$-th \pb within this segment has $S_{i,j}$ parallelism strategies. 
We model the size of profiling space, i.e., number of parallel programs that need to be compiled and profiled as:

\vspace{-1mm}
\begin{align}
    \sum_{i=1}^{N}{(\prod_{j=1}^{K_i} S_{i,j} + \sum_{j=1}^{N} \sum_{(l, k) \in D_{i,j}}{S_{i,l}*S_{j, k}})} 
\end{align}
\noindent
where $D_{i, j}$ is a list containing pairs of index $(l, k)$ of {\pb}s that have cross-segment tensor dependencies within segment $i, j$.
The left side of the summation represents the number of parallelism strategies combinations for all {\pb}s within a segment, while the right side is the number of parallelism strategy combinations for cross-segment dependent \pb pairs.

In the worst case, where the entire model acts as a single distinct segment, the number of programs that need to be compiled and profiled is $\prod_{j=1}^{M}{S_{j}}$, which is the simple combination of the parallelism strategies of $M$ {\pb}s, as explained in Section~\ref{SearchSpace}.
In the best case, where the model consists of a single distinct segment repeated, and the cross-segment tensor dependencies only occur between the first and last \pb within it, the profiling space is $\prod_{i=j}^{K} S_{j} + S_{1}*S_{K}$, i.e., the sum of all parallelism strategies for the K {\pb}s within a single segment, plus the resharding from the last \pb to the first \pb.

Thanks to the extensive use of repeated model structures and wide range of parallelism-preserving subgraphs in existing models,  
the number of distinct segments and the {\pb}s per segment remains within a reasonable range.
For example, after grouping two BMM operators in self-attention into a single \pb, the repeated transformer layer in GPT model has only 4 {\pb}s, corresponding to four matrix multiplication operators.
As a result, we can evaluate the costs of all global parallelism plans by profiling just a few hundred short parallel programs.

Running programs multiple times incurs a significant time overhead, depending on the training workload and the execution efficiency of the parallelism plans.
In addition, the compilation time for parallel programs can also be substantial, especially when the computation graph is long but training workload is light-weight.
To further mitigate the overhead, \sysname introduces two optimizations:
First, it enforces a dynamic profiling time budget, which is continuously updated based on the fastest observed parallelism plans, aggressively trimming the profiling of inefficient or stalled executions.
Second, it parallelizes the compilation of different programs and overlaps the compilation phase with the profiling phase.

\vspace{-1mm}
\subsection{Plan Cost Estimation and Optimization}
We represent a global parallelism plan as a tuple $\mathbf{i} = (i_1, i_2, \dots, i_N)$, where $i_n$ denotes selecting the $i_n$-th parallelism plan for the $n$-th segment in a model with $N$ segments.
We estimate its execution time $T(\mathbf{i})$ and memory consumption $M(\mathbf{i})$ using profiles of distinct segments.
For the $n$-th segment that selects the $i_n$-th parallelism plan, we denote $p_n(i_n)$ as the computation time, $c_n(i_n)$ as the communication time, and $m_n(i_n)$ as the peak memory usage.
For each adjacent pair of segments $(n, n+1)$, the resharding cost when using the $i_n$-th and $i_{n+1}$-th parallelism plan is denoted as $r_n(i_n, i_{n+1})$.
The total execution cost and memory usage are defined as:

\begin{equation}
T(\mathbf{i}) = \sum_{n=1}^{N} (p_n(i_n) + c_n(i_n)) + \sum_{n=1}^{N-1} r_n(i_n, i_{n+1})
\end{equation}

\begin{equation}
M(\mathbf{i}) = \sum_{n=1}^{N} m_n(i_n)
\end{equation}

The first term in \( T(\mathbf{i}) \) aggregates segment computation and communication costs, while the second term sums the cross-segment resharding overheads.
Each part of the cost calculation is extracted from the profile of distinct segments, ultimately combining to represent the overall cost of the global parallelism plan $\mathbf{i}$.

%\sysname estimates the execution cost and memory consumption of a global parallelism plan by aggregating the computation cost, communication cost, and resharding overheads of all segments, derived from the profiles of the corresponding distinct segments.

%Each component of the cost and memory consumption is derived from the profiles of the distinct segments. %The memory consumption is calculated in a similar manner.

\sysname searches for the plan with the minimal execution cost under the constraint of the memory usage limit, which is formulated as a dynamic programming problem.
%It formulates the global plan selection as a dynamic programming problem, where each segment chooses a parallelism plan to minimize the total cost. 
It first builds a cost table and a memory table for each segment’s possible plans, based on the profiles of the distinct segments.
Then, starting from the first segment in the computation graph, the algorithm recursively explores all feasible combinations of segment plans, accounting for segment cost, cross-segment resharding cost, and accumulated memory consumption.
To reduce the complexity of the dynamic programming, we quantize the memory usage of each parallelism plan.

This segment-based cost combination method not only reuses segment costs to reduce profiling overhead, but also allows flexible parallelism plan selection.
Segments (even those of the same type) may adopt different plans: some high-throughput but memory-intensive, others low-throughput but memory-efficient, maximizing overall throughput while staying near the memory limit.
%Even among matched segments, some may use high-throughput but memory-intensive plans, while others adopt low-throughput but memory-efficient plans, maximizing throughput while staying near the memory limit.

% Note that this segment-based cost combination method not only allows reusing segment costs to reduce profiling overhead, but also enables flexible use of different parallelism plans for the same type of model segments. 
% For multiple fingerprint-matched segments, some may utilize a high-throughput but memory-intensive plan. Others may instead adopt a low-throughput but memory-efficient plan, maximizing model throughput while staying as close as possible to the memory usage limit.



==> CFP-VLDB-arxiv-v2/content/RelatedWorks.tex <==
\vspace{-3mm}
\section{Related Works}

\textbf{Modeling the Intra-operator Parallelism Search Space.}
% Many works~\cite{xu2021gspmd, dtensor, yuan2022oneflow} offer concise yet comprehensive methods to express tensor partitioning, accommodating various parallel paradigms. 
Many works~\cite{xu2021gspmd, dtensor, yuan2022oneflow} propose concise yet expressive tensor partitioning methods that support diverse parallel paradigms. More recently, strategies that partition the temporal dimension have been used~\cite{summa_parallel, primpar_eurosys24, distal_pldi22, distribute_mapping_tensor_compute_sc23} to further expand the intra-operator parallelism space.
% \textcolor{blue}{
%  FlexFlow\cite{lu2017flexflow} introduce an abstraction for parallel a operator named as SOAP (Sample-Operator-Attribute-Parameter), however, it relies on the specific meanings of an operator's data dimensions, thus lacking in universality. GSPMD\cite{xu2021gspmd} offers a concise yet comprehensive method to express tensor partitioning, accommodating various large model parallel paradigms. 
%  PyTorch DistributedTensor (DTensor)\cite{dtensor} is an API for prototyping with distributed tensor primitives, simplifying distributed computing creation in an SPMD paradigm.
%  OneFlow\cite{yuan2022oneflow} offers an abstraction model for describing model partitioning called SBP.
% }
% Recently, parallelism strategies that partition temporal dimension for operators have been adopted by several parallel systems~\cite{summa_parallel, primpar_eurosys24, distal_pldi22, distribute_mapping_tensor_compute_sc23} to expand the intra-operator parallelism search space.
% Some works~\cite{overlapping_google_asplos23, overlapping_t3_asplos24, overlapping_centauri_asplos24, superscaler_supporting_flexible_dnn} discussed the scheduling space of after tensor partitioning, which favored overlapping communication and computation to hide communication overhead.

\textbf{Automatic Search for Intra-operator Parallelism.} 
% To efficiently search for intra-operator parallelism plans, most works, including ToFu~\cite{tofu2019}, TensorOpt~\cite{cai2021tensoropt}, PaSE~\cite{pase},AccPar~\cite{accpar}, HAP~\cite{hap_heter_gpu_spmd_eurosys24}, and PrimPar~\cite{primpar_eurosys24}, have employed various symbolic cost models and dynamic programming-based search algorithms.
To efficiently search for intra-operator parallelism plans, most works~\cite{tofu2019, cai2021tensoropt, pase, accpar, hap_heter_gpu_spmd_eurosys24, primpar_eurosys24}, have employed various symbolic cost models and dynamic programming-based search algorithms.
FlexFlow~\cite{lu2017flexflow} and Automap~\cite{schaarschmidt2021automap} used a Monte Carlo-based search algorithm and employed an ML-based approach to evaluate plans.
Colossal-Auto~\cite{liu2023colossal} and Alpa~\cite{zheng2022alpa} use an ILP solver to find the plan with the lowest communication volume.
Some works~\cite{aceso_eurosys24, uniap} also adopt profile-based approaches, profiling operators and communication primitives separately and aggregating the results into cost models.
However, this operator-level profiling approach still struggles to capture execution efficiency accurately.
Moreover, they mainly focus on stage-level pipeline partitioning and rely on predefined intra-operator parallel templates, rather than fully exploring the space.

% Our work demonstrates that the intra-operator parallelism search space can be reduced to considering only a few {\pb}s and model segments, thus enabling the use of real runtime metrics as the cost model for optimizing parallelism plans.

\textbf{Combine Intra- and Inter-operator Parallelism.}
Many frameworks adopt fixed parallelism plans per pipeline stage, without exploring the intra-operator search space~\cite{narayanan2019pipedream, NEURIPS2021_piper, huang2019gpipe}.
% Alpa~\cite{zheng2022alpa} explores intra-operator parallelism and pipeline parallelism in two separate stages and maps them to device layers based on communication characteristics.
Aceso~\cite{aceso_eurosys24} combines the exploration of intra-operator and pipeline parallelism by using reconfiguration mechanisms to alleviate performance bottlenecks.
Galvatron~\cite{galvatron} proposes a decision-tree abstraction to decompose multi-level parallelism, and also uses a symbolic cost model to search for the optimal parallelism plan.
nnScaler~\cite{nnscaler} offers scheduling abstractions that let experts define flexible search spaces. It leverages existing search strategies to explore the reduced search space and generate parallelism plans, e.g., Alpa for intra-operator parallelism and Tessel~\cite{tessel} for pipeline parallelism.

% \textcolor{blue}{
% SuperScaler\cite{superscaler_supporting_flexible_dnn} decouples the model
% partitioning, scheduling, and data dependency preserving, allowing for more flexible expression of parallel plans. 
% This supports specialized parallelization plan for emerging DNN modelss, such as AlphaFold and Swin-Transformer.
% }

% \textcolor{blue}{
% \textbf{Compiler IR and DSLs for Tensor Parallelism.}
% DistIR\cite{santhanam2021distir} uses an MLIR-based\cite{mlir} representation for describing distributed tensor programs in MPMD form. 
% AutoMap\cite{schaarschmidt2021automap} introduces PartIR for expressing tensor partitioning at the IR level of the XLA compiler, provides a Python interface for specifying partitioning of certain operators, and proposes a rewriting engine to fully partition the entire program.
% }










==> content/Conclusion.tex <==
\section{Conclusion}
%\sysname currently does not consider multi-dimensional partition and temporal dimension partition. 
%These partitioning methods further expand the tensor parallel search space and may lead to higher computation and communication efficiency.
%Our future work will focus on using profile-based methods to identify multi-level parallel plans, including pipeline parallelism, seeking end-to-end parallel training solutions for large models that closely align with optimal real-world performance while maintaining reasonable search time.

This paper introduces \sysname, a system that search intra-operator parallelism configurations by leveraging runtime profiles of actual parallel programs. 
The key idea is to profile a limited space by identifying a new structure named \pb, which is a group of operators enjoying communication-free tensor partition propagation.
An optimal tensor partition of operators within a \pb should be inferred from the partition of input tensor through partition propagation to avoid additional communication.
Thus, it is sufficient to profile each \pb with different input tensor partitions.
On GPT, LLAMA, and MoE models, \sysname achieves up to a 1.51x, 1.31x, and 3.43x performance improvement over the state-of-the-art framework, Alpa. 

